Same Root Different Leaves: Time Series and Cross-Sectional Methods in Panel Data

A central goal in social science is to evaluate the causal effect of a policy. One dominant approach is through panel data analysis in which the behaviors of multiple units are observed over time. The information across time and space motivates two general approaches: (i) horizontal regression (i.e., unconfoundedness), which exploits time series patterns, and (ii) vertical regression (e.g., synthetic controls), which exploits cross-sectional patterns. Conventional wisdom states that the two approaches are fundamentally different. We establish this position to be partly false for estimation but generally true for inference. In particular, we prove that both approaches yield identical point estimates under several standard settings. For the same point estimate, however, each approach quantifies uncertainty with respect to a distinct estimand. In turn, the confidence interval developed for one estimand may have incorrect coverage for another. This emphasizes that the source of randomness that researchers assume has direct implications for the accuracy of inference.

==> content/covariates.tex <==
\section{Beyond Panel Data} \label{sec:covariates}
%
%The purpose of this section is to contextualize our findings in settings beyond panel data. 
%
%% COVARIATES 
%\subsection{Estimation and Inference with Covariates} 
%
We depart from panel data to a setting with both outcomes and covariates.
%
For cohesiveness, we continue with the Basque study but now consider a different dataset, the details of which are provided in \cite{abadie1} and \cite{synthR}. 
%
Specifically, for each region $i$, we observe (pretreatment) covariates $\bx_i \in \Rb^{T_0}$, 
which includes per-capita GDP (the outcome variable), as well as population density, sectoral production, investment, and human capital (the auxiliary predictor variables) all prior to the onset of terrorism. 
%
Focusing on the single treated period setting, we denote $Y_i$ as the observed GDP for the $i$th region one year after the onset of terrorism. 
%
Let $\bX = [\bx_i: i \le N_0]$ and $\by = [Y_i: i \le N_0]$ denote the matrix of covariates and vector of outcomes for the control regions, respectively. 
%
In line with the rest of this article, our interest is to predict Basque Country's GDP in the absence of terrorism, $Y_N(0)$. 

\smallskip
\noindent
{\bf Two general solutions.} 
%
This is a well studied problem in the causal inference literature. 
%
Among the numerous existing methodologies, we discuss two prominent approaches. 
%

\smallskip
\noindent
{\em I: Covariate adjustment.} 
%
One classical approach is known as covariate adjustment. 
%
At a high level, covariate adjustment posits a (linear) relationship between outcome variables and covariates that is stable across units. 
%
Methodologically, this is carried out by regressing the control regions' treated period GDPs, $\by$, on the control regions' covariates, $\bX$; the learned regression coefficients are then applied to Basque Country's covariates, $\bx_N$, to predict 
Basque Country's GDP in the absence of terrorism. 
%
 
\smallskip
\noindent
{\em II: Synthetic controls.} 
%
Synthetic controls has also emerged as a popular tool. 
%
Philosophically, synthetic controls posits a relationship between treated and control units that is stable across covariates and outcome variables. 
%
Methodologically, this is carried out by regressing Basque Country's covariates, $\bx_N$, on the control regions' covariates, $\bX'$; the learned regression coefficients are then applied to control regions' treated period GDPs, $\by$, to predict 
Basque Country's GDP in the absence of terrorism. 
%

\smallskip
\noindent
{\em An ``obvious'' connection.} 
%
Recalling our earlier notation and mapping $\bx_N$ to $\by_N$, $\bX$ to $\bY_0$, and $\by$ to $\by_T$, we identify covariate adjustment and synthetic controls as simply \HZ~and \VT~regression, respectively. 
%
Therefore, Theorem~\ref{thm:equivalent} asserts that if the regression weights are learned via estimators within the symmetric class, then the two methods produce numerically identical estimates for $Y_N(0)$. 
%
Theorem \ref{thm:inference.hz_vt} then states that valid inference relies on cross-sectional patterns and a linear relationship between outcomes and covariates. 
%
Conceptually, this suggests that synthetic controls and covariate adjustment are two sides of the same coin.   
%
As a result, we can interpret covariate adjustment through the lens of synthetic controls and vice versa. 

%% GENERAL OLS 
%\subsection{General Linear Regression} 
%%
%We step out of the causal inference frame of reference to look at the problem of linear regression in generality, whereby panel data and learning with covariates are special instances. 
%%
%Theorem~\ref{thm:inference.hz_vt} states that the statistical uncertainty of the out-of-sample prediction is governed by two distinct sources of randomness: 
%(i) the construction of the regression model from the in-sample data,
%and
%(ii) the similarity between the in- and out-of-sample data. % as measured through the $\ell_2$-metric. 
%%
%Standard OLS uncertainty estimators, which correspond to \HZ~and \VT~specific intervals in panel studies, account for the first source of randomness. 
%%
%They are rigorous when the design matrix is full column rank. 
%%They are rigorous only when the design matrix is full column rank, as is typically assumed in the canonical OLS literature. 
%%
%By contrast, the mixed OLS interval is derived without the canonical full column rank assumption or restrictions on the data configuration. 
%%
%Accordingly, it incorporates both sources of randomness and thus, generalizes the standard OLS interval.  
%%
%%In this view, it generalizes the standard OLS interval. 
%%
%In this view, our results in Section~\ref{sec:inference} build upon the broader OLS literature, particularly in the high-dimensional regime, which may be of independent interest. 
%

%The uncertainty from the former corresponds to the misspecification of the linear model while the uncertainty of the latter corresponds to the $\ell_2$-d


%As such, this work builds upon the general OLS literature, which may be of independent interest. 






==> content/diagnostic.tex <==
% DIAGNOSTIC 
\subsection{Learning from the Mistakes of Others}
\label{sec:diagnostic} 
%
As highlighted in Section~\ref{sec:problem}, the confidence intervals derived for each approach only depends on its particular in-sample error, though the other approach's error remains informative for the chosen approach. 
% 
This motivates an alternative natural proposition to the mixed confidence interval of Section~\ref{sec:ci.2}: for a given regression direction, use the other direction's in-sample error as a diagnostic to examine the validity of Assumptions~\ref{assump:hz} and \ref{assump:vt} (iv.b). 
%
More formally, we define the following statistics: 
%
\begin{align} \label{eq:tau} 
	\tau^\hz(\by_N, \bY_0) &= \frac{ \| \bH^{(v)}_\perp \by_N \|^2_2} { \| \by_N \|^2_2} 
	\quad \text{and} \quad 
	\tau^\vt(\by_T, \bY_0) = \frac{ \| \bH^{(u)}_\perp \by_T \|^2_2} { \| \by_T \|^2_2}.  
\end{align} 
%
The numerators of $\tau^\hz(\by_N, \bY_0)$ and $\tau^\vt(\by_T, \bY_0)$ are the \VT~and \HZ~in-sample errors, respectively. 
%
We use $\tau^\hz(\by_N, \bY_0)$ to determine if $(\by_N, \bY_0)$ obeys Assumption~\ref{assump:hz} (iv.b), and use $\tau^\vt(\by_T, \bY_0)$ to determine if $(\by_T, \bY_0)$ obeys Assumption~\ref{assump:vt} (iv.b). 
% 
From this perspective, $\tau^\hz$ and $\tau^\vt$ can serve as a first line of defense to identify out-of-sample inputs, e.g., $\by_N$ for \HZ~regression, that will be difficult for $\bhalpha$ and $\bhbeta$ to predict. 
% 

Given \eqref{eq:tau}, it is natural to ask how we determine which inputs are flagged? 
%
By construction, $\tau^\hz$ and $\tau^\vt$ take values within the interval $[0,1]$. 
%
If $\by_N \in \text{rowspan}(\bY_0)$, then $\tau^\hz(\by_N, \bY_0) = 0$, otherwise $\tau^\hz(\by_N, \bY_0) > 0$. 
%
Similarly, if $\by_T \in \text{colspan}(\bY_0)$, then $\tau^\vt(\by_T, \bY_0) = 0$, otherwise $\tau^\vt(\by_T, \bY_0) > 0$. 
% 
However, we may not wish to be so strict on using zero as a hard threshold. 
%
Instead, given that $1 - \tau^\hz$ and $1 - \tau^\vt$ are similar to the standard $R^2$ metric used in regression analyses, we can transfer the same principles used to determine ``acceptable'' $R^2$ scores to our setting of interest. 

Crucially, we underscore that $\tau^\hz \approx 0$ and $\tau^\vt \approx 0$ do {\em not} suggest that the $(N,T)$th predictions will necessarily be accurate. 
%
These values only reduce our uncertainty in conditions (i.a) and (iv.b)---no more no less. 
%
Indeed, there still remains other potential sources of uncertainty, i.e., other conditions may be violated without our knowledge. 
% 
To fully determine the suitability of \HZ~or \VT~regression towards a given dataset, we would ideally examine the validity of each aspect of their posited DGPs. 
%
Currently, only a subset of the conditions in Assumptions~\ref{assump:hz} and \ref{assump:vt} are commonly checked. 
%
As discussed, condition (i.a) is traditionally evaluated through the chosen direction's in-sample error. 
% 
Conditions (ii) and (iii) are commonly investigated through residual analyses, though they cannot ever be fully verified. 
%
Conditions (i.b) and (iv.a) involve unobservable quantities that make it arduous if not impossible to furnish data driven metrics.  
%
In light of this, we advocate treating $\tau^\hz$ and $\tau^\vt$ as one-sided tests: if $\tau^\hz \approx 1$ or $\tau^\vt \approx 1$, then we should be cautious about our out-of-sample prediction as our uncertainty in the overall composition of assumptions has only increased. 

% comparison with literature 
{\bf Comparison with the literature.}  
%
To the best of our knowledge, similar metrics have remained largely absent in the literature, likely because traditional frameworks have not explored condition (iv) in great depth. 
%
Below, we discuss connections with the few related works in the causal inference literature. 

% SI 
\underline{\em I: \cite{si}.} 
%
Our proposed statistics presented in \eqref{eq:tau} are motivated by the subspace inclusion statistic of \cite{si}.  
%
More specifically, \cite{si} introduces $\tau^\vt(\by_T, \bY_0)$ to check if Assumption~\ref{assump:vt} (iv.b) holds in practice. 
%
Notably, \cite{si} focuses purely on \VT~regression. 
%
As such, \cite{si} do not consider $\tau^\hz(\by_N, \bY_0)$. 
%
A key aspect of this work is the observation that \HZ~regression implicitly relies on cross-sectional correlations and \VT~regression implicitly relies on time series correlations. 
%
Therefore, just as \cite{si} introduces $\tau^\vt(\by_T, \bY_0)$ as a useful metric for \VT~regression, this work introduces $\tau^\hz(\by_N, \bY_0)$ as a useful metric for \HZ~regression. 


% King-Zeng 
\underline{\em II:  \cite{king_zeng_2006}.} 
%
To facilitate this comparison, consider \HZ~regression. 
% 
Similar to the focus of this section, \cite{king_zeng_2006} set out to provide a useful measure to guide researchers in identifying causal estimands that can be answered. 
%
In our context, the authors argue that $\bhalpha$ can be safely applied to $\by_N$ if $\by_N$ is embedded within the convex hull of $\bY_0$, i.e., there exists weights $\bw$ satisfying $\bw \succeq \bzero$, $\bone' \bw =1$, and $\by_N = \bY_0 \bw$. 
%
Despite their different derivations, the convex hull metric and \eqref{eq:tau} are based on the same concept: they both relate the prediction quality of $\hY^\hz_{NT}(0) = \langle \by_N, \bhalpha \rangle$ to the distance between $\by_N$ and $\bY_0$. 
%
The key difference is the notion of distance, specifically interpolation versus extrapolation. 
%
\cite{king_zeng_2006} defines datapoints lying within the convex hull as interpolation and those lying outside as extrapolation. 
% 
The authors claim that extrapolation is generally more hazardous than interpolation, albeit without formal arguments. 
% 
In contrast, we assert that extrapolation is a theoretically sound condition, provided it is considered in conjunction with the other conditions laid out in Assumptions~\ref{assump:hz} and \ref{assump:vt} and not in a vacuum. 
%
We further argue that \eqref{eq:tau} is more robust than the convex hull metric. 
%
To see this, note that if $\by_N$ lies within the convex hull of $\bY_0$, then for every $i \le N_0$, $\by_i = [Y_{it}: t \le T_0]$ (the $i$th row of $\bY_0$) necessarily falls outside the convex hull of $\{\by_N, \by_1, \dots, \by_{i-1}, \by_{i+1}, \dots, \by_{N_0}\}$.  
%
Put another way, if the $i$th and $N$th units swapped roles (i.e., unit $i$ receives treatment and unit $N$ remains under control), then the convex hull test would pass in one case and fail in the other, even though the same data is considered in both tests. 
%
This highlights the convex hull metric's sensitivity to the permutation of in-and out-of-sample datapoints. 

% Comparison with mixed interval 
{\bf Comparison with the mixed confidence interval.} 
%
We consider $(\tau^\hz, \tau^\vt)$ relative to $\hv_0$. 
%
Although $(\tau^\hz, \tau^\vt)$ can serve as useful metrics for regression analyses, we argue that $\hv_0$ is generally more favorable for two primary reasons:
%
(i) while $\hv_0$ couples the \HZ~and \VT~errors into one uncertainty estimator, $(\tau^\hz, \tau^\vt)$ decouples the two errors into two separate stages thereby maintaining the separation of \HZ~and \VT~regressions; 
(ii) the utility of $(\tau^\hz, \tau^\vt)$ relies on a subjective threshold while the parameter associated with the nominal coverage for $\hv_0$ is well-defined. 
%
For these reasons, we advocate for the usage of $\hv_0$ over $(\tau^\hz, \tau^\vt)$. 


==> content/discussion.tex <==
\section{Discussion} \label{sec:discussion} 
%
The purpose of this section is to discuss key implications of our results stated in Sections~\ref{sec:estimation} and \ref{sec:inference}. 

% Regularization
\subsection{The Practitioner's Guide to Panel Data}
%
\begin{center}
{\em
	``In general, how do we decide between \HZ~and \VT~regressions?''
} 
\end{center}    
% 
A widely accepted rule-of-thumb is to choose the regression based on the configuration of the data. 
%
Often, there is limited information in one form or another, which lends the problem to a particular approach.
% 
More concretely, \HZ~and \VT~approaches are cautioned against when $T \gg N$ and $N \gg T$, respectively. 
%
However, \cite{mc_panel} argues that regularization allows the two approaches to be simultaneously applicable for the same setting, which then enables a more systematic comparison.
% between the two approaches. 
%
Despite this assertion, \VT~methods continue to be, by and large, the leading approach for most panel data studies.  
%

%As established in Section~\ref{sec:inference}, one primary takeaway of this article is   
% 
%At the same time, Section~\ref{sec:estimation} classifies standard regression formulations into two classes. 
%
%For one class of formulations, the two approaches derive numerically identical point estimates; in the other class, the two approaches derive different point estimates in general. 
%% 
%Arguably, the former class of symmetric formulations offers one notion of interpretability since the same point estimate can be explained from two different perspectives. 

This article offers a new perspective that departs from the standard principles discussed above. 
%
To arrive at our viewpoint, we recall two important observations. 
%
First, Section~\ref{sec:estimation} establishes that under one class of regression formulations, the \HZ~and \VT~approaches yield numerically identical point estimates. 
%
Second, Section~\ref{sec:inference} proves that both time series and cross-sectional correlations can play a critical role for valid inference.   
%
Collectively, these results suggest the following guideline: 
%
\begin{center} 
{\em 
unless there is strong evidence (perhaps informed through domain knowledge) in support of considering only one correlation pattern, a panel data practitioner should choose a regression formulation that preserves estimation equivalence and use a joint confidence interval to quantify their uncertainty. 
}
\end{center} 
%
In doing so, the practitioner no longer needs to debate between the two approaches since the same counterfactual estimate can be derived from both perspectives---thus, offering one notion of interpretability---and the uncertainties in both correlation patterns are measured. 
% 
Under this protocol, we now ask which regression formulation should be adopted? 

At first glance, OLS may seem to be a natural candidate. 
%
To begin, OLS excludes hyperparameters, which can be advantageous for practitioners since hyperparameters induce more degrees of freedom and thus potential subjectivity. 
%
In recent years, OLS has also been shown to demonstrate ``benign overfitting'' in high-dimensional settings with surprisingly strong theoretical properties \citep{ols1, ols3, ols2}, i.e., OLS generalizes well on out-of-sample data despite overfitting to in-sample data. 
% 
However, in limited data regimes, it can be worrisome to rely on OLS, as displayed in Figures~\ref{fig:teaser_est} and \ref{fig:basque}. 
%
Consequently, PCR and ridge emerge as attractive compromises. 
%
Both methods are also closely linked to OLS and to each other. 
%
Namely, ridge converges to the OLS minimum $\ell_2$-norm solution as the penalty term tends to zero, while PCR performs OLS in the reduced subspace spanned by the top principal $k$ components. 
%
Ridge can also be viewed as a ``smooth'' variant of PCR: 
in ridge, higher order singular values are largely unaffected by the penalty term while the lower order singular values are heavily penalized; in PCR, the higher order singular values are kept as is while the lower order singular values are removed entirely. 
%
Unlike ridge, however, PCR allows for inference and further enables the HRK variance estimator, which is unbiased, to be valid. 
%
For these reasons, we can refine our prescription to elevate PCR as the benchmark formulation. 
%
We refer the interested reader to \cite{pcr, pcr2} for a detailed theoretical analysis of PCR. 

%hus, should be regarded as a salient feature much like sparsity. 

% in this article, we establish that both perspectives r necessary for valid inference 
% at same time, there r some formulations that preserve estimation equivalence while others break it 
% we argue that symmetry is a form of interpretability (one notion) 
% should be regarded as a salient feature much like sparsity has historically been desired 

% from this perspective, our results suggest that unless there is strong evidence (perhaps guided by domain knowledge) in support of focusing on a single correlation pattern, then a practitioner may benefit from choosing a regression formulation from the equivalence class and to use joint CI (treat both equally) 
% in choosing an estimator from this class--w/o intercept--and using our proposed joint confidence interval, a practitioner does not have to deliberate between \HZ~and \VT~regression since the same counterfactual estimate is yielded from both regressions and the uncertainties in both correlation patterns are reflected in the confidence interval. 
% less subjectivity, one less degree of freedom 

% given this, how do we decide b/w three? 
% OLS may be natural candidate: no hyperparameter (less subjectivity) 
% nice theoretical properties 
% however, as shown in Figure, may struggle in presence of limited data 
% use regularization: pcr and ridge similar to OLS
% also similar to each other
% however, PCR has several advantages: allows for inference + can use HRK variance estimator, which is unbiased 
% thus, a more refined prescription is to use PCR + joint CI  


% DOUBLY ROBUST
{\bf Doubly Robust Estimators.} %\label{sec:doubly_robust}  
%
Within the panel data setting, there are two important works on doubly robust estimation 
%These past few years have seen a surge of doubly robust estimators
 that also attempt to remove the burden of deliberating between \HZ~and \VT~regressions: 
%
%Within our setting of interest, there are two important works: 
the synthetic difference-in-difference~(\SDID) estimator of \cite{sdid} and the augmented \SC~(\ASC) estimator of \cite{sc_aug}.  
%
\SDID~combines \HZ~and \VT~regression with \DID. 
%
In our setting, its prediction for the missing $(N,T)$th entry can be written as 
%
\begin{align}  
	\hY^\sdid_{NT}(0) &= \sum_{i < N} \hbeta_i Y_{iT} + \sum_{t < T} \halpha_t Y_{Nt}  -\sum_{i < N} \sum_{t < T} \hbeta_i \halpha_t Y_{it}  
	\\ &=  \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhbeta, \bY_0 \bhalpha \rangle, \label{eq:sdid}
\end{align} 
%
where $\bhalpha$ and $\bhbeta$ represent general \HZ~and \VT~regression weights, respectively.  
%
To help readers gain an intuition for \eqref{eq:sdid}, \cite{sdid} notes that $\bhalpha = 1/(T-1) \bone$ and $\bhbeta = 1/(N-1) \bone$ recovers \DID. 
%
Moving beyond simple \DID~to performing a weighted two-way bias removal, the authors propose to learn $\bhalpha$ via \eqref{eq:hz.cvx.1} with $\lambda = 0$ and $\bhbeta$ via \eqref{eq:vt.cvx.1} with $\lambda > 0$. 
%

The \ASC~estimator uses an outcome model to correct the bias induced by the \SC~estimator. 
% 
In particular, the \ASC~estimator predicts the $(N,T)$th missing potential outcome as 
%
\begin{align}
\hY^\asc_{NT}(0) &= 
\hM_{NT}(0) + \sum_{i < N} \hbeta_i (Y_{iT} - \hM_{iT}(0)), 
\label{eq:ascm}
\end{align} 
%
where $\hM_{iT}(0)$ is the estimator for the $(i,T)$th potential outcome. 
% 
In \cite{sc_aug}, the authors instantiate $\hM_{iT}(0)$ with a \HZ~regression outcome model:  
%
\begin{align}
	\hM_{iT}(0) &= \sum_{t < T} \halpha_t Y_{it} = \langle \by_i, \bhalpha \rangle, \label{eq:hz_outcome} 
\end{align}
%
where $\by_i = [Y_{it}: t < T]$. 
%
Plugging \eqref{eq:hz_outcome} into \eqref{eq:ascm} gives  
%
\begin{align}
	\hY^\asc_{NT}(0) &= \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhbeta, \bY_0 \bhalpha \rangle. 
\end{align} 
%
Notably, this variant of \ASC~takes the same form as \SDID, as seen in \eqref{eq:sdid}. 
%
In contrast to \cite{sdid}, \cite{sc_aug} learns $\bhalpha$ via \eqref{eq:hz.rr.1} with $\lambda_1 = 0$ and $\lambda_2 > 0$, and $\hbeta$ via \eqref{eq:vt.cvx.1} with $\lambda = 0$. 

We attempt to gain a deeper understanding of \SDID~and \ASC~with \HZ~regression adjustment by studying their prediction properties under the OLS and PCR settings. 
%
\begin{theorem} \label{thm:sdid} 
%
Consider \ESDID~and \EASC~with $\bhalpha$ and $\bhbeta$ as the OLS solutions to \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1}, respectively, with $\lambda_1 = \lambda_2 = 0$.
%
If $\bhalpha$ and $\bhbeta$ are the minimum $\ell_2$-norm solutions, 
then $\ESDID = \EASC = \EHZ = \EVT$, i.e., 
%
\begin{align}
	\hY^\esdid_{NT}(0) = \hY^\easc_{NT}(0) = \hY^\ehz_{NT}(0) = \hY^\evt_{NT}(0) 
	= \langle \by_N, \bY_0^\dagger \by_T \rangle 
    	= \sum_{\ell=1}^R (1/s_\ell) (\by'_N \bv_\ell) (\bu'_\ell \by_T).
\end{align} 
%
Next, consider $\bhalpha$ and $\bhbeta$ as the PCR solutions to \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1}, respectively, with $\lambda_1 = \lambda_2 = 0$ and $\bY_0^{(k)}$ for $k < R$ in place of $\bY_0$.
%
If $\bhalpha$ and $\bhbeta$ are the minimum $\ell_2$-norm solutions, 
then $\ESDID = \EASC = \EHZ = \EVT$, i.e., 
%
\begin{align}
	\hY^\esdid_{NT}(0) = \hY^\easc_{NT}(0) = \hY^\ehz_{NT}(0) = \hY^\evt_{NT}(0)
	= \langle \by_N, (\bY_0^{(k)})^\dagger \by_T \rangle 
    	= \sum_{\ell =1}^k (1/s_\ell) (\by'_N \bv_\ell) (\bu'_\ell \by_T).
\end{align} 
%
\end{theorem} 
%
Theorem~\ref{thm:sdid} states that the unconstrained and unregularized variants of \SDID~and \ASC~%with \HZ~regression adjustment 
each reduce to \HZ~OLS, which is equivalent to \VT~OLS as per Theorem~\ref{thm:equivalent}. 
%
As a result, a practitioner in favor of either doubly robust estimator who learns the \HZ~and \VT~weights via OLS will inevitably arrive at the same point estimate as a practitioner who simply utilizes \HZ~or \VT~OLS. 
%
The same reduction and storyline holds for PCR.   
%uses either doubly robust estimator and learns the \HZ~and \VT~weights via OLS or PCR will inevitably arrive at the same point estimate as 
%
However, Theorem~\ref{thm:sdid} does not hold in general for other penalized regressions including ridge. 




% SC 
\subsection{Beyond Panel Data} 
%
Let us take a detour from panel data to a setting with both outcomes and covariates.
%
As a concrete example, consider a clinical trial with $N$ patients, $T-1$ covariates, and $1$ trial period, amounting to $T$ measurements per patient. 
%
Let $\bx_i \in \Rb^{T-1}$ represent patient $i$'s covariates (e.g., age, gender, blood pressure), which are collected prior to the trial. 
%
We denote $Y_i \in \Rb$ as the clinical outcome under placebo during the trial period for the $i$th patient. 
%
Let $\bX = [\bx_i: i < N]$ and $\by = [Y_i: i < N]$ denote the matrix of covariates and vector of placebo outcomes for the first $N-1$ patients, respectively. 
%
In line with the rest of this article, our interest is to predict the clinical outcome under placebo for the $N$th patient, $Y_N$, who is assigned to the treatment arm. 
%
A classical method is to regress $\by$ on $\bX$ and apply the regression weights on $\bx_N$ to predict $Y_N$. 
%
This is known as covariate regression adjustment, which posits that the outcomes are a linear function of the covariates. 

\SC~offers an alternative methodological strategy to estimate $Y_N$. 
%
In particular, \SC~methods regress $\bx_N$ on $\bX'$ and apply the regression weights on $\by$ to predict $Y_N$. 
%
By mapping $\bx_N$ to $\by_N$, $\bX$ to $\bY_0$, and $\by_T$ to $\by$, we immediately identify that covariate regression adjustment and \SC~are simply \HZ~and \VT~regression, respectively, in disguise. 
%
Therefore, our results in Section~\ref{sec:estimation} indicate that if the regression weights are learned via OLS, PCR, or ridge, then covariate regression adjustment and \SC~produce numerically identical estimates for $Y_N$. 
%
Theorem \ref{thm:inference.hz_vt} takes it another step further by establishing that valid inference requires cross-sectional correlation patterns and a linear relationship between the outcomes and covariates. 
%
%Theorem \ref{thm:inference.hz_vt} takes it another step further by establishing that the two approaches, when viewed in harmony, converge to the same asymptotic distribution. 
%
Conceptually, this means that \SC~is equivalent to covariate regression adjustment! 
%
As a result, we can interpret covariate regression adjustment through the lens of \SC~and vice versa. 
% 
By extension, we further conclude that the synthetic interventions estimator of \cite{si}, which generalizes \SC~to multiple interventions, is numerically equivalent to conducting separate covariate regression adjustments for each intervention, i.e., the mapping from covariates to outcomes depends on the intervention associated with the outcome. 
%




==> content/equivalence_2.tex <==
\section{Finite-Sample Point Estimation} \label{sec:estimation} 
%
We begin our exploration of the connections between \HZ~and \VT~regressions 
%with a re-examination of the relation between \HZ~and \VT~regressions 
with respect to finite-sample point estimation under several notable settings in the literature. 
%
To facilitate our discussion, we denote the singular value decomposition (SVD) of $\bY_0$ as 
\begin{align}
    \bY_0 &= \sum_{i =1}^{R} s_i \bu_i \bv_i',
\end{align}
%
where $\bu_i \in \Rb^{N-1}$ and $\bv_i \in \Rb^{T-1}$ are the left and right singular vectors, respectively, $s_i \in \Rb$ are the ordered singular values, and $R = \text{rank}(\bY_0) \le \min\{N-1, T-1\}$. 
%
Let $\bU \in \Rb^{(N-1) \times R}$ and $\bV \in \Rb^{(T-1)\times R}$ be the matrices formed by the left and right singular vectors, respectively, and $\bS \in \Rb^{R \times R}$ as the diagonal matrix of ordered singular values. 
%
Therefore, $\bY_0 = \bU \bS \bV'$. 
%
We define the Moore-Penrose pseudoinverse of $\bY_0$ as 
%
\begin{align}
	\bY_0^\dagger &= \sum_{i=1}^R (1/s_i) \bv_i \bu_i', 
\end{align} 
or, equivalently, $\bY_0^\dagger = \bV \bS^{-1} \bU'$. 
%
In what follows, we say $\HZ = \VT$ if the \HZ~and \VT~regressions arrive at the same prediction value and $\HZ \neq \VT$ otherwise.
%, i.e., their respective predictions may differ from one another depending on the setting of interest. 

% LEAST SQUARES 
\subsection{Least Squares} 
%
We first analyze \HZ~and \VT~regressions of the following formulations: 
%
\begin{itemize}
	\item [(a)] \HZ~Regression:  for $\lambda_1, \lambda_2 \ge 0$, 
	\begin{align} 
		&\bhalpha = \argmin_{\balpha} ~\| \by_T - \bY_0 \balpha \|_2^2 ~+~ \lambda_1 \| \balpha \|_1 ~+~ \lambda_2 \|\balpha \|_2^2 \label{eq:hz.rr.1} 
		\\ &\hY_{NT}^\hz(0) = \langle \by_N, \bhalpha \rangle. \label{eq:hz.rr.2} 
	\end{align} 
	
	\item [(b)] \VT~Regression: for $\lambda_1, \lambda_2 \ge 0$, 
	\begin{align} 
		&\bhbeta = \argmin_{\bbeta} ~\| \by_N - \bY'_0 \bbeta \|_2^2 ~+~ \lambda_1 \| \bbeta \|_1 ~+~ \lambda_2 \| \bbeta \|_2^2 \label{eq:vt.rr.1} 
		\\ &\hY_{NT}^\vt(0) = \langle \by_T, \bhbeta \rangle. \label{eq:vt.rr.2} 
	\end{align} 
\end{itemize} 
%
Below, we study the relative behaviors of \HZ~and \VT~regressions for various choices of $\lambda_1$ and $\lambda_2$. 

% Unconstrained OLS 
\subsubsection{Ordinary Least Squares} \label{sec:unregularized} 
%
Our investigation commences with the setting of ordinary least squares (OLS), where $\lambda_1 = \lambda_2 = 0$. 
%
%Within the panel data literature, one important work that uses the OLS estimator for program evaluation is that of \cite{hcw}. 
%
In Theorem~\ref{thm:ols} below, we present a result that is simple, perhaps even obvious, from a technical point of view, but can be highly nonintuitive from a conceptual level as it contradicts conventional wisdom in the literature. 
%
\begin{theorem} \label{thm:ols} 
%
Consider OLS with $\lambda_1 = \lambda_2 = 0$. 
%
If $\bhalpha$ and $\bhbeta$ are the unique minimum $\ell_2$-norm solutions, then 
%Consider four settings: 
%(a) $\bhalpha$ is the unique minimum $\ell_2$-norm solution;
%(b) $\by_N \in \emph{rowspan}(\bY_0)$;
%(c) $\bhbeta$ is the unique minimum $\ell_2$-norm solution;
%(d) $\by_T \in \emph{colspan}(\bY_0)$. 
%%
%Suppose any of the following pair of settings holds: 
%(a,c),  
%(a,d), 
%(b,c), 
%or 
%(b,d).  
%%
%%condition (i): (a) and (c); 
%%condition (ii): (a) and (d); 
%%condition (iii): (b) and (c); 
%%or 
%%condition (iv): (b) and (d);
%%holds, 
%Then 
$\EHZ = \EVT$. 
%
In particular,  
%
\begin{align} \label{eq:ols} 
    \hY_{NT}^{\ehz}(0) &= \hY_{NT}^{\evt}(0) 
    = \langle \by_N, \bY_0^\dagger \by_T \rangle 
    = \sum_{i =1}^R (1/s_i) (\by'_N \bv_i) (\bu_i' \by_T).
\end{align}
\end{theorem} 
%%(i) \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1} correspond to the unique solutions with minimum $\ell_2$-norm,
%or (ii)  $\by_N \in \emph{rowspan}(\bY_0)$ and $\by_T \in \emph{colspan}(\bY_0)$, 
%
Theorem~\ref{thm:ols} establishes that \HZ~and \VT~OLS regressions yield identical pointwise predictions, regardless of the sizes of $N$ and $T$. 
%
Therefore, a practitioner that uses \VT~regression to impute the missing $(N,T)$th entry will arrive at the same prediction value had she taken a \HZ~regression approach instead, and vice versa. 
%
%Such a statement may come across surprising 
This is an unfamiliar conception when juxtaposed with standard beliefs in the literature. 
%
Historically, the relative magnitudes of $N$ and $T$ have not only largely dictated the choice between \HZ~and \VT~regression, but also motivated the need for regularization \citep{sc_enet, abadie_hour, mc_panel}. 
% 
%Expanding on the former, it has been noted in the literature that \HZ~(unconfoundedness) and \VT~(synthetic controls) approaches do not work well when $T \gg N$ and $N \gg T$, respectively. 
% 
Notably, \cite{mc_panel} writes 
%
\begin{center}
	{\em ``The horizontal and vertical regressions are fundamentally different approaches, and they cannot easily be nested. Without some form of regularization they cannot be applied in the same setting, because the nonregularized versions require
$N > T$ or $N < T$, respectively. As a result there is also no
direct way to test the two methods against each other. Given a particular choice for regularization, however, one can use cross-validation methods to compare the two approaches.''} 
\end{center} 
%
Although Theorem~\ref{thm:ols} opposes this claim, the above quote is not without some merit. 
%
Indeed, it is well known that OLS is ill-defined when $\bY_0$ is rank deficient. 
% 
However, among the infinitely many solutions in this scenario is the minimum $\ell_2$-norm solution, which possesses several attractive properties. 
%
First, it is the unique solution that is entirely embedded within the rowspace of the ``covariate'' matrix, i.e., $\bY_0$ for \HZ~regression and $\bY'_0$ for \VT~regression. 
%
This solution is arguably sufficient for valid statistical inference since any element in the nullspace of the covariate matrix is mapped to zero. 
%
Moreover, the minimum $\ell_2$-norm solution emerges when an unregularized, undetermined least squares problem (e.g., \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1} with $\lambda_1=\lambda_2=0$) is optimized using gradient descent, a ubiquitous optimizer in practice. 
% 
This phenomena is an example of ``implicit regularization'', where the optimization algorithm is biased towards a particular global minima (solution), even though the bias is not explicit in the objective function or problem formulation. 
%
A critical mystery discovered by deep learning methodology is that deep neural networks that are trained without any explicit regularization, even in high-dimensional settings where the number of parameters exceeds the sample size, have been observed to demonstrate ``benign overfitting'', i.e., they generalize well on out-of-sample data despite overfitting to the in-sample data \citep{ireg2, ireg3, ireg4, ireg1, ireg5}. 
%
Such prediction models are known as interpolators. 
%
Recent works have studied OLS in the high-dimensional regime and shown it to be a minimum norm interpolator with surprisingly good theoretical properties \citep{ols1, ols3, ols2}. 
%
Since generalization in our context corresponds to counterfactual predictions, it may be worth revisiting the role of implicit regularization and interpolators in panel data settings and causal inference more generally. 

%
%We now discuss condition (ii) of Theorem~\ref{thm:ols}. 
%%
%We first argue that condition (ii) is natural when $N \gg T$ or $T \gg N$. 
%%
%To see this, observe that when $N \gg T$, then $\bY_0$ likely has full column rank, which not only implies $\by_N$ necessarily lies within the rowspace of $\bY_0$ but also $\bhalpha$ is the minimum $\ell_2$-norm solution since the solution is now unique. 
%%
%Similarly, when $T \gg N$, then $\bY_0$ likely has full row rank, which implies $\by_T$ necessarily lies within the columnspace of $\bY_0$ and $\bhbeta$ is the minimum $\ell_2$-norm solution. 
%%
%Note that the above settings immediately enforce $\bhalpha$ and $\bhbeta$ to be the minimum $\ell_2$-norm solutions, i.e., condition (i) is implied by.
%%
%We also take this opportunity to remind the reader that the former and latter data configurations correspond to the typical \HZ~and \VT~regression settings, respectively. 
%% 


\begin{remark}
Within the panel data literature, OLS has been analyzed in program evaluation in numerous works, including \cite{hcw, li_bell, li2020}. 
%Within the panel data literature, one important work that uses the \emph{OLS} estimator for program evaluation is that of \cite{hcw}. 
\end{remark} 

% PCR 
\subsubsection{Principal Component Regression} 
%
Next, we consider a close variant of OLS known as principal component regression (PCR) \citep{pcr_jolliffe}. 
%
PCR first finds a $k$ dimensional representation of the covariate matrix via principal component analysis (PCA), a standard linear dimensionality reduction method; then, PCR performs OLS using the compressed $k$ dimensional covariates.  
%
Equivalently, \cite{pcr} showed that PCR can be interpreted as performing (hard) singular value thresholding, a well-studied matrix completion algorithm \citep{donoho14, usvt1, usvt2}, on the covariate matrix followed by OLS. 
%
To present our statement, let 
%
\begin{align} \label{eq:rank_k} 
	\bY_0^{(k)} = \sum_{i=1}^k s_i \bu_i \bv_i'
\end{align}
%
denote the rank $k < R$ approximation of $\bY_0$ that retains the top $k$ principal components. 
% 
%Within the synthetic controls literature, \cite{si} proposes a PCR estimator when $\bY_0$ exhibits low rank structure. 
%
We now state our results for PCR in Corollary~\ref{cor:pcr}, which follows immediately from Theorem~\ref{thm:ols}. 
%
% corollary pcr 
\begin{cor} \label{cor:pcr} 
%
Consider Theorem~\ref{thm:ols} with $\bY_0^{(k)}$ for any $k < R$ in place of $\bY_0$. 
%
Then $\EHZ = \EVT$.  
%
In particular, 
%
\begin{align} \label{eq:pcr} 
    \hY_{NT}^{\ehz}(0) &= \hY_{NT}^{\evt}(0) 
    = \langle \by_N, (\bY_0^{(k)})^\dagger \by_T \rangle 
    = \sum_{i =1}^k (1/s_i) (\by'_N \bv_i) (\bu_i' \by_T).
\end{align}
\end{cor} 
%
In words, Corollary~\ref{cor:pcr} states that PCR upholds the symmetry between \HZ~and \VT~regression approaches, provided the same number of principal components $k$ is used in both settings. 

\begin{remark}
Within the \ESC~literature, \cite{rsc, mrsc, si} utilize PCR to construct synthetic comparison groups when $\bY_0$ exhibits low rank structure. 
\end{remark} 

% Regularization
\subsubsection{Regularized Least Squares} \label{sec:regularized} 
%
Next, we consider various forms of regularized regression that are widely used and analyzed in the literature. 
%
We reemphasize that regularized forms of \HZ~and \VT~regression appear to have been largely motivated by the misconception that either unregularized \HZ~or \VT~regression---{\em never} both---is valid when $N \neq T$. 
%
To examine this notion, we do not place any assumptions on the relative sizes of $N$ and $T$. 
%%

% examine final statement of quote about cross validation 

% Ridge
\paragraph{Ridge Regression.} %\label{sec:rr} 
%
Consider ridge regression (also known as Tikhonov regularization), where $\lambda_1=0$ and $\lambda_2 > 0$ \citep{ridge}.  
%
As aforementioned, a rank deficient $\bY_0$ often discourages the usage of OLS since the gram matrix (i.e., $\bY'_0 \bY_0$ for \HZ~regression and $\bY_0 \bY'_0$ for \VT~regression) is ill-conditioned. 
%
In these settings, ridge provides a remedy by adding a {\em ridge} on the diagonal of the gram matrix (e.g., $\bY'_0 \bY_0 + \lambda_2 \bI$), which increases all eigenvalues by $\lambda_2$, thus removing the problem of non-invertibility. 
%
Put another way, when $\lambda_2 > 0$, the criterion in \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1} are strictly convex so the solutions are unique. 
%

\begin{theorem} \label{thm:ridge} 
%
Consider ridge regression with $\lambda_1 = 0$ and any $\lambda_2 > 0$. 
%
Then $\EHZ = \EVT$. 
%
In particular, 
%
\begin{align} \label{eq:ridge} 
    \hY_{NT}^{\ehz}(0) &= \hY_{NT}^{\evt}(0) 
    = \langle \by_N,  (\bY_0' \bY_0 + \lambda_2 \bI)^{-1} \bY_0' \by_T \rangle 
    = \sum_{i =1}^R \frac{s_i}{s_i^2 + \lambda_2} (\by'_N \bv_i) (\bu_i' \by_T).
\end{align}
\end{theorem} 
%
As with OLS and PCR, \HZ~and \VT~ridge regressions also arrive at the same prediction. 
%
Therefore, symmetry between \HZ~and \VT~approaches is preserved under ridge for the same value of $\lambda_2$. 
%
This is expected given that the Moore-Penrose pseudoinverse can be defined as  
%
\begin{align} \label{eq:limits} 
    \bY_0^\dagger = \lim_{\lambda \rightarrow 0} (\bY_0' \bY_0 + \lambda \bI)^{-1} \bY_0' = \lim_{\lambda \rightarrow 0} \bY_0' (\bY_0 \bY_0' + \lambda \bI)^{-1}. 
\end{align} 
%
We finish by noting that \eqref{eq:ridge} does not hold when \HZ~and \VT~ridge select different penalty values of $\lambda_2$. 

\begin{remark}
Within the \ESC~literature, \cite{sc_aug} explore the properties of a doubly robust estimator that utilizes \EHZ~ridge regression. 
\end{remark} 

% Lasso
\paragraph{Lasso Regression.} %\label{sec:lasso} 
%
Another form of regularization is lasso regression, where $\lambda_1 > 0$ and $\lambda_2 = 0$ \citep{lasso1, lasso2}. 
%
Along with ridge, lasso has received enormous amounts of attention in the statistics literature and has become a popular tool for estimating linear coefficients in high-dimensional regimes, particularly when seeking sparse solutions. 
%
Unlike ridge regression, the lasso criterion in \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1} are convex but not  strictly convex. 
%
As such, there is either a unique solution or infinitely many solutions.
%
Therefore, for this part of the section only, we make a mild assumption that the entries of $\bY_0$ are drawn from a continuous distribution. % on $\Rb^{(N-1) \times (T-1)}$. 
%
As established in \cite{lasso_ryan}, this guarantees that the lasso solution is unique, regardless of the sizes of $N$ and $T$. 
%
\begin{theorem} \label{thm:lasso} 
%
Consider lasso regression with any $\lambda_1 > 0$ and $\lambda_2 = 0$. 
%
Then $\EHZ \neq \EVT$. 
\end{theorem} 
%
Theorem~\ref{thm:lasso} establishes that lasso breaks the symmetry between \HZ~and \VT~approaches, even for the same choice of $\lambda_1$. 
%
As a result, for different choices of $\lambda_1$ (the more plausible scenario in practice), \HZ~and \VT~lasso are likely to disagree as well. 
%\HZ~and \VT~lasso may also disagree for different choices of $\lambda_1$, which is the more plausible scenario in practice. 

\begin{remark}
Several notable works in the \EVT~regression and \ESC~literatures, e.g., \cite{li_bell, arco, sc_lasso1}, explore and analyze lasso regression. 
\end{remark}  


% Elastic-net
\paragraph{Elastic Net Regression.} %\label{sec:enet} 
%
Mixing both $\ell_1$ and $\ell_2$-penalties, i.e., $\lambda_1, \lambda_2 > 0$, is known as elastic net regression \citep{enet}. 
%
As noted in \cite{hastie}, elastic net selects variables similar to the lasso, but deals with correlated variables more gracefully as with ridge.
%
When $\lambda_2 > 0$, the elastic net criterion is strictly convex, which gives rise to a unique solution. 
%
\begin{theorem} \label{thm:enet} 
%
Consider elastic net regression with any $\lambda_1, \lambda_2 > 0$. 
%
Then $\EHZ \neq \EVT$. 
\end{theorem} 
%
Theorem~\ref{thm:enet} establishes that \HZ~and \VT~elastic net predictions are not equivalent in general, even for the same $(\lambda_1, \lambda_2)$ pair. 
%
Therefore, differing penalty terms between \HZ~and \VT~will likely break the symmetry as well. 
%
Theorem~\ref{thm:enet} is to be expected given the presence of lasso within elastic net. 
%
\begin{remark}
In \cite{sc_enet}, the authors propose the elastic net regression variant of the original \ESC~method. 
\end{remark} 

% CVX
\subsection{Convex Regression} \label{sec:cvx} 
%
Next, we consider an important version of constrained regression that restricts the regression weights to be nonnegative and sum to one: 
%
\begin{itemize}
	\item [(a)] \HZ~Regression: for $\lambda \ge 0$, 
	\begin{align} 
		&\bhalpha = \argmin_{\balpha} ~\| \by_T - \bY_0 \balpha \|_2^2 ~+~ \lambda \| \balpha \|_2^2 \quad \text{subject to} \quad \balpha' \bone = 1, \balpha \succeq \bzero \label{eq:hz.cvx.1} 
		\\ &\hY_{NT}^\hz(0) = \langle \by_N, \bhalpha \rangle. \label{eq:hz.cvx.2} 
	\end{align} 
	
	\item [(b)] \VT~Regression: for $\lambda \ge 0$, 
	\begin{align} 
		&\bhbeta = \argmin_{\bbeta} ~\| \by_N - \bY_0' \bbeta \|_2^2 ~+~ \lambda \| \bbeta \|_2^2 \quad \text{subject to} \quad \bbeta' \bone = 1, \bbeta \succeq \bzero \label{eq:vt.cvx.1} 
		\\ &\hY_{NT}^\vt(0) = \langle \by_T, \bhbeta \rangle. \label{eq:vt.cvx.2} 
	\end{align} 
\end{itemize} 
%
We refer to this class of least square problems as convex regression. 
%
Traditionally, standard convex regression formulations set $\lambda = 0$. 
%
In our formulation, we include the $\ell_2$ penalty because $\lambda = 0$ can induce multiple minima \citep{sc_enet, abadie_hour, sdid}.
%\footnote{Notably, in their presentation of their synthetic difference-in-differences (\SDID) estimator, which combines both horizontal and vertical regression, \cite{sdid} also includes an $\ell_2$ penalty term in their \VT~convex regression problem. In practice, they also recommend including the $\ell_2$ penalty term in their \HZ~convex regression problem to yield a unique solution.}  
%
With $\lambda > 0$, the criterion becomes strictly convex, which gives rise to a unique solution. 
%
Therefore, we state our result with the $\ell_2$ penalty term vanishing to zero. 
%
\begin{theorem} \label{thm:cvx}
Consider convex regression with $\lambda \rightarrow 0^+$. 
%
Then $\EHZ \neq \EVT$. 
\end{theorem}
%
Theorem~\ref{thm:cvx} states that \HZ~and \VT~convex regression are not equivalent in general. 
%
This is an intuitive result that can be seen through an extreme scenario in which \HZ~and \VT~convex regressions select a single most predictive pretreatment period and control unit, respectively. 
%
In such a setting, the treated unit's outcome during the most predictive pretreatment period (as determined by \HZ~convex regression) need not be in congruence with the treated period outcome associated with the most predictive control unit (as determined by \VT~regression). 
%
To make this concrete, consider $N=T$ with $\bY_0 = \bI$, $\by_N = \be_i$, and $\by_T = 2 \be_i$, where $\be_i$ is the canonical basis vector whose $i$th coordinate is $1$. 
%
Here, $\bhalpha = \bhbeta = \be_i$, yet $\hY^\hz_{NT}(0) = 1$ and $\hY^\vt_{NT}(0) = 2$.  
%
\begin{remark}
Convex regression has been studied extensively within the \ESC~literature \citep{abadie1, abadie2, abadie4, abadie_hour, abadie_survey, ferman_pinto} and has also been analyzed in \EHZ~regression \citep{sdid}. 
\end{remark} 

% DOUBLY ROBUST
\subsection{Doubly Robust Estimators} \label{sec:doubly_robust}  
%
These past few years have seen a surge of doubly robust estimators. 
%
Within our setting of interest, there are two important works: the synthetic \DID~(\SDID) estimator of \cite{sdid} and the augmented \SC~(\ASC) estimator of \cite{sc_aug}.  
%
At its core, \SDID~combines \HZ~and \VT~regression with \DID. 
%
In our setting, its prediction for the missing $(N,T)$th entry can be written as 
%
\begin{align}  
	\hY^\sdid_{NT}(0) &= \sum_{i < N} \hbeta_i Y_{iT} + \sum_{t < T} \halpha_t Y_{Nt}  -\sum_{i < N} \sum_{t < T} \halpha_t \bhbeta_i Y_{it}  
	\\ &=  \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhalpha, \bY_0' \bhbeta \rangle, \label{eq:sdid}
\end{align} 
%
where $\bhalpha$ and $\bhbeta$ represent general \HZ~and \VT~regression weights, respectively.  
%
To help readers gain an intuition for \eqref{eq:sdid}, \cite{sdid} notes that $\bhalpha = 1/(T-1) \bone$ and $\bhbeta = 1/(N-1) \bone$ recovers \DID. 
%
Moving beyond simple \DID~to performing a weighted two-way bias removal, the authors propose to learn $\bhalpha$ via \eqref{eq:hz.cvx.1} with $\lambda = 0$ and $\bhbeta$ via \eqref{eq:vt.cvx.1} with $\lambda > 0$. 
%

The \ASC~estimator uses an outcome model to correct the bias induced by the \SC~estimator. 
% 
In particular, the \ASC~estimator predicts the $(N,T)$th missing potential outcome as 
%
\begin{align}
\hY^\asc_{NT}(0) &= 
%\sum_{i < N} \hbeta_i Y_{iT} + \hM_{NT}(0) - \sum_{i < N} \hbeta_i \hM_{iT}(0) 
\hM_{NT}(0) + \sum_{i < N} \hbeta_i (Y_{iT} - \hM_{iT}(0)), 
%\sum_{t < T} \bhalpha_t Y_{Nt}  -\sum_{i < N} \sum_{t < T} \bhalpha_t \bhbeta_i Y_{it}  
\label{eq:ascm}
\end{align} 
%
where $\hM_{iT}(0)$ is the estimator for the $(i,T)$th potential outcome. 
% 
In \cite{sc_aug}, the authors instantiate $\hM_{iT}(0)$ with a \HZ~regression outcome model:  
%
\begin{align}
	\hM_{iT}(0) &= \sum_{t < T} \halpha_t Y_{it} = \langle \by_N, \bhalpha \rangle. \label{eq:hz_outcome} 
\end{align}
%
Plugging \eqref{eq:hz_outcome} into \eqref{eq:ascm} then gives  
%
\begin{align}
	\hY^\asc_{NT}(0) &= \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhalpha, \bY_0' \bhbeta \rangle. 
\end{align} 
%
Notably, this variant of \ASC~takes the same form as \SDID, as seen in \eqref{eq:sdid}. 
%
However, \cite{sc_aug} learns $\bhalpha$ via \eqref{eq:hz.rr.1} with $\lambda_1 = 0$ and $\lambda_2 > 0$, and $\hbeta$ via \eqref{eq:vt.cvx.1} with $\lambda = 0$. 


We attempt to gain a deeper understanding of the robustness properties of both \SDID~and \ASC~with \HZ~regression adjustment by removing all structural constraints imposed on the regression weights. 
%
That is, we analyze the two estimators under the OLS setting, where $\bhalpha$ and $\bhbeta$ are learned via \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1}, respectively, with $\lambda_1 = \lambda_2 = 0$. 
%
\begin{theorem} \label{thm:sdid} 
%
Consider \ESDID~and \EASC~with $\bhalpha$ and $\bhbeta$ as the OLS solutions to \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1}, respectively, with $\lambda_1 = \lambda_2 = 0$.
%
%If (i) \eqref{eq:hz.rr.1} and \eqref{eq:vt.rr.1} correspond to the unique solutions with minimum $\ell_2$-norm 
%or (ii) $\by_N \in \emph{rowspan}(\bY_0)$ and $\by_T \in \emph{colspan}(\bY_0)$, 
If $\bhalpha$ and $\bhbeta$ are the unique minimum $\ell_2$-norm solutions, 
then $\ESDID = \EASC = \EHZ = \EVT$. 
%
In particular,  
%
\begin{align}
	\hY^\esdid_{NT}(0) = \hY^\easc_{NT}(0) = \langle \by_N, \bY_0^\dagger \by_T \rangle 
    = \sum_{i =1}^R (1/s_i) (\by'_N \bv_i) (\bu_i' \by_T).
\end{align} 
\end{theorem} 
%
In the absence of any regularization or constraints, Theorem~\ref{thm:sdid} states that \SDID~and \ASC~with \HZ~regression adjustment are actually equivalent to \HZ~regression, which itself is equivalent to \VT~regression, as per Theorem~\ref{thm:ols}. 
%
Therefore, both estimators lose their double robustness properties. 
%
We conclude by noting that Theorem~\ref{thm:sdid} also holds for PCR, but does not hold in general for other penalized regressions including ridge. 

% KERNELS
\subsection{Kernel Extensions} 
%
{\color{blue} 
A natural question at this juncture is whether the results stated above hold when the regression formulations are kernelized, i.e., models are learned in an arbitrary feature space. 
%
We argue that, in general, our guarantees no longer hold. 
%
To see this, consider \HZ~regression. 
%
Let $\phi: \Rb^{T-1} \rightarrow \Hc$ be a mapping from the original space to the reproducing kernel Hilbert space (RKHS), $\Hc$. 
%
Let $\Phi(\bY_0)$ be the ``matrix'' of features whose $i$th row is given by $\phi(\by_i)$, where $\by_i = [Y_{it}: t < T]$. 
%
To generalize the objective functions discussed in this section to the kernel setting, we replace all instances of $\bY_0$ and $\bY'_0$ with $\Phi(\bY_0)$ and $\Phi(\bY'_0)$, respectively. 
%
Crucially, $\Phi(\bY_0)' \neq \Phi(\bY'_0)$ in general. 
% 
The two are, however, equivalent for the linear kernel (used in this section), which defines $\Hc$ to be the original space. 
%
} 







==> content/guide2.tex <==
\section{The Researcher's Guide to Panel Data} \label{sec:guide} 
%
\smallskip 
\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black]
	\begin{center}
	{
		{\bf Q2:} ``How do we decide between \HZ~and \VT~regressions?'' 
	} 
	\end{center} 
\end{tcolorbox}
% 

% current approaches 
\subsection{Current Approaches} 
%
% data configuration 
\noindent
{\bf Data configuration principle.} 
%
A widely accepted rule-of-thumb is to choose the regression based on the configuration of the data. 
%
Often, there is limited information in one form or another, which lends the problem to a particular approach.
% 
Concretely, \HZ~and \VT~are cautioned against when $T \gg N$ and $N \gg T$, respectively \citep{abadie4, sc_enet, li_bell, mc_panel}. 
%
However, \cite{mc_panel} argues that regularization allows the two approaches to be simultaneously applicable for the same setting, which then enables a more systematic comparison.
%
Nevertheless, \VT~methods continue to be the leading approach for panel data studies across many literatures.  
%

% doubly robust 
\smallskip
\noindent
{\bf Doubly robust estimation.}
% 
A second popular response is to remove the burden of deciding altogether. 
% 
This is an old idea that dates back to the difference-in-differences (\DID) estimator \citep{did1}, 
%\citep{did1, did2, did3, did4}, 
which is still widely used in applied economic research today.
%
At a high level, \DID~posits an additive outcome model with unit- and time-specific fixed effects, known more colloquially as the ``parallel trends'' assumption. 
%
The recent work of \cite{sdid} anchors on the \DID~principle and brings in concepts from the unconfoundedness and synthetic controls literatures to derive a doubly robust estimator called synthetic difference-in-differences (\SDID). 
%
In our setting, the \SDID~prediction for the missing $(N,T)$th entry can be written as 
%
\begin{align}  
	\hY^\sdid_{NT}(0) &= \sum_{i \le N_0} \hbeta_i Y_{iT} + \sum_{t \le T_0} \halpha_t Y_{Nt}  -\sum_{i \le N_0} \sum_{t \le T_0} \hbeta_i \halpha_t Y_{it}  
	\\ &=  \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhbeta, \bY_0 \bhalpha \rangle, \label{eq:sdid}
\end{align} 
%
where $\bhalpha$ and $\bhbeta$ represent general \HZ~and \VT~models, respectively.  
%
The authors note that $\bhalpha = (1/T_0) \bone$ and $\bhbeta = (1/N_0) \bone$ recovers \DID. 
%
Moving beyond simple \DID~to performing a weighted two-way bias removal, the authors propose to learn $\bhalpha$ via simplex regression and $\bhbeta$ via simplex regression with an $\ell_2$-penalty. %

Another notable work is that of \cite{sc_aug}. 
%
The authors introduce the augmented synthetic control (\ASC) estimator, which uses an outcome model to correct the bias induced by the classical synthetic controls estimator. 
% 
Concretely, the \ASC~estimator predicts the $(N,T)$th missing potential outcome as 
%
\begin{align}
	\hY^\asc_{NT}(0) &= 
	\hM_{NT}(0) + \sum_{i \le N_0} \hbeta_i (Y_{iT} - \hM_{iT}(0)), \label{eq:ascm}
\end{align} 
%
where $\hM_{iT}(0)$ is the estimator for the $(i,T)$th entry. 
% 
The authors instantiate %$\hM_{iT}(0)$ as 
%
\begin{align}
	\hM_{iT}(0) &= \sum_{t \le T_0} \halpha_t Y_{it}. % = \langle \by_i, \bhalpha \rangle, 
	\label{eq:hz_outcome} 
\end{align}
%
%where $\by_i = [Y_{it}: t \le T_0]$ for any $i \le N$. 
%
Plugging the \HZ~outcome model in \eqref{eq:hz_outcome} into \eqref{eq:ascm} then gives   
%
\begin{align} \label{eq:asc_hz} 
	\hY^\asc_{NT}(0) &= \langle \by_T, \bhbeta \rangle +  \langle \by_N, \bhalpha \rangle - \langle \bhbeta, \bY_0 \bhalpha \rangle. 
\end{align} 
%
We consider this particular variant of \ASC, which takes the same form as \SDID, as seen in \eqref{eq:sdid}. 
%
In contrast to \cite{sdid}, \cite{sc_aug} learns $\bhalpha$ via ridge regression and $\bhbeta$ via simplex regression. 
%
Given their rising popularities, we look to gain a deeper understanding of both approaches by studying their estimation characteristics when 
$(\bhalpha, \bhbeta)$ are learned via OLS and PCR. 
%
\begin{cor} \label{cor:sdid} 
%
$\ESDID = \EASC = \EHZ = \EVT$ for 
(i) $(\bhalpha, \bhbeta)$ as the OLS minimum $\ell_2$-norm solutions
and 
(ii) $(\bhalpha, \bhbeta)$ as the PCR solutions with the same choice of $k < R$. 
%
\end{cor} 
%
Somewhat surprisingly, Corollary~\ref{cor:sdid} states that a researcher who uses the unregularized variants of \SDID~and \ASC~inevitably arrive at the same point estimate as their colleague who simply uses \HZ~or \VT~OLS. 
%
The same phenomena occurs for PCR. 
%
From this, we observe that \SDID~and \ASC~lose their weighted double-differencing effects under certain formulations. 
%
However, Corollary~\ref{cor:sdid} is not to discredit either approach. 
%
%A significant draw to both methods is the ability to naturally and simultaneously encode knowledge of time and unit specific structures into the estimator. 
The fact remains that both methods allow researchers to naturally and simultaneously encode their knowledge of time and unit specific structures into the estimator. 
%
\SDID~and \ASC~warrant further studies and careful consideration. 
%deserve to be studied in detail and considered carefully.  

% OUR APPROACH
%\subsection{Our Approach---Agnostic Regression} 
\subsection{Our Approach---Panel Data Agnostic (\panda) Regression} 
%
To answer Q3, we summarize two insights derived in this article: 
%
(i) \HZ~and \VT~regressions yield numerically identical estimates under several formulations;   
%
(ii) time series and cross-sectional correlations play critical roles for valid inference.  
%
In this view, both \HZ~and \VT~perspectives deserve our appreciation and attention. 
%
Neglecting either side can lead to misinformed conclusions, as showcased in Section~\ref{sec:joint_advantage}. 
%
Thus, this article challenges the one-approach-fits-all mindset that is trending in several fields. 
%
It also discourages the biased attitude towards asymmetric formulations without justifiable cause as they implicitly establish a hierarchy between the two approaches. 
%
%In many applications, the most suitable approach and formulation is not known a priori. 
%With the hope of changing the narrative, 
%With the hope of shifting the landscape,
%To begin moving away from these practices, 
With the hope of changing course, 
this article offers an alternative perspective: 
%
\smallskip 
\begin{center}
	{\em if the DGP is unknown, then the researcher should be agnostic.}
\end{center} 
\smallskip 
%
The core philosophy of \panda~regression is to advocate for the coexistence of both regressions when there is little to no evidence that suggests one correlation pattern is more meaningful than the other. 
%
We translate philosophy into practice through a (i) symmetric estimator and (ii) mixed confidence interval. 
%
\panda~regression, therefore, relieves the burden of deliberation placed on the researcher---the same counterfactual estimate is derived from both perspectives and the uncertainty associated with each perspective is accounted for. 
%
In this view, \HZ~and \VT~regressions are not {\em dueling} perspectives but {\em dual} perspectives. 

% symmetric estimator 
\smallskip
\noindent
{\bf Best practices.} 
Through the lens of model checking, we discuss the two facets of \panda~regression to construct principles for best practice. 
%

% symmetric estimator 
\smallskip
\noindent
{\em I: Symmetric estimator.} 
%
In many applications, it is not known a priori which estimator to use. 
%
Systematic comparisons such as cross-validation and stability analyses are effective instruments for such cases \citep{pcs, mc_panel}.  
%
If these evaluations do not motivate a particular formulation, then we recommend PCR. 
%
To arrive at this viewpoint, we compare the symmetric estimators. 

%
OLS is an attractive candidate since it excludes hyperparameters, which induce more degrees of freedom and thus subjectivity. 
%
However, applying OLS in limited data regimes can lead to erroneous outcomes, as illustrated in Figure~\ref{fig:teaser_est}. 
%
PCR and ridge can overcome this drawback through regularization. 
%
%Both methods are also connected to OLS and to each other.  
Both methods are also connected to one another.  
%
Ridge can be viewed as a ``smooth'' variant of PCR: 
in ridge, higher order singular values are largely unaffected by the penalty while the lower order singular values are heavily penalized; in PCR, the higher order singular values are untouched while the lower order singular values are removed entirely. 
%
Since conducting inference for ridge can be challenging \citep{ridge_dsw}, 
%Since it is arguably easier to conduct inference for PCR than ridge, 
we elevate PCR as the benchmark. 
%
We refer the interested reader to \cite{pcr, pcr2} for detailed analyses of PCR. 

% MIXED CI 
\smallskip
\noindent
{\em II: Mixed confidence interval.} 
%
As argued in Section~\ref{sec:joint_advantage}, our mixed confidence interval exhibits desirable robustness properties relative to \HZ~and \VT~specific intervals.  
%
The aim of this discussion, however, is {\em not} to promote our specific method but to motivate future methods to account for both sources of randomness rather than just one. 
%
In fact, $\hv_0$ is unlikely to be optimal given that it is an artifact of our assumed DGP and choice of analysis. 
%
There are numerous other approaches with differing philosophies on the sources of randomness, each with their unique merits.  
% 
Extensive model checking, therefore, is critical to identify the most suitable approach for a given problem. 
%
%The purpose of this discussion is to motivate future methods to account for both sources of randomness rather than just one. 
%%
%We hope this article serves as a stepping stone in this new direction. 

%%is generally advantageous over \HZ~and \VT~specific intervals. 
%e.g., 
%design-based permutation inference \citep{abadie1, abadie2, abadie4, sc_enet, ferman_pinto_inf, guido_inf},
%time series-based permutation inference \citep{sc_lasso1},
%cross-sectional-based permutation inference \citep{shaikh_toulis},
%prediction intervals \citep{cattaneo},
%and large-sample approximations under correct specification \citep{li2020, si}. 

% remark
\begin{remark} 
%
Model checks cannot validate an analysis, but they can reveal problems. 
%
Thus, the checks may suggest that linear predictors are ill-suited 
and none of the \HZ, \VT, or mixed intervals are valid. 
%warrant consideration. 
%
\end{remark}

%%
%\begin{remark}
%The discussion above is central to the class of linear predictors. 
%%
%If the data exhibits strong nonlinearity, then nonlinear predictors would naturally be more suitable. 
%\end{remark} 

% With all things “equal”, (eg same reported errors) we believe our guideline is reasonable. In spirit of OC cams razor where simplicity in this context is symmetry. Lean towards simplicity, 


==> content/illustration.tex <==
\newpage 

\section{Empirical Illustrations} \label{sec:illustration} 
%
In this section, we provide details on the Basque study that were absent in the main article. 
%
We also revisit two other canonical case studies from the synthetic controls literature: California's Proposition 99 \citep{abadie2} and West Germany Reunification \citep{abadie4}. 
%
Our objective is twofold: (i) confirm our estimation results of Section~\ref{sec:estimation} and (ii) apply our confidence intervals constructed in Section~\ref{sec:inference}. 

% BASQUE
\subsection{Terrorism in Basque Country} 

% background 
{\bf Background.} 
%
The purpose of this study is to examine the impact of terrorism on Basque Country's economy. 
%
This dataset consists of $N = 17$ Spanish regions, including Basque Country, whose per capita GDPs are collected from 1955--1998 yielding $T = 43$ years. 
%
Basque Country is our single treated region, which we will label as the $N$th region; the remaining regions act as our control regions. 
%
The first wave of terrorist activity in 1970 represents the treatment. 
%
Thus, the pre- and post-intervention durations are $15$ and $28$ years, respectively. 
%
Our outcome variable of interest is the per capita GDP. 
%
In our attempt to isolate the economic cost of terrorism on Basque Country, we set out to estimate its counterfactual GDP growth in the absence of terrorism, i.e., $Y_{Nt}(0)$ for $t \in [1970, 1998]$. 
%
Notice that our causal estimand is no longer a single point, but rather a time series of $28$ years. 
%
We will apply the estimators provided in Section~\ref{sec:estimation} to estimate the counterfactual GDP in each year with the following inputs at our disposal: 
%
Basque Country's pre-intervention GDP trajectory, $\by_N \in \Rb^{15}$;  
the control regions' pre-intervention GDP trajectories, $\bY_0 \in \Rb^{16 \times 15}$; 
and the control regions' GDPs during the post-intervention year $t$, $\by_t \in \Rb^{16}$ for $t \in [1970, 1998]$. 

% estimation 
{\bf Estimation.} 
%
We display the counterfactual predictions associated with the estimators of Section~\ref{sec:estimation} in Figure~\ref{fig:basque}. 
%
For visual purposes, we present the symmetric regressions---OLS, PCR, ridge---in Figure~\ref{fig:basque_symmetric} and the asymmetric regressions---lasso, elastic net, and simplex---in Figure~\ref{fig:basque_asymmetric}. 
%
We use the default \texttt{scikit-learn} hyperparameters ($\lambda_1, \lambda_2$) for the regularized regressions. 
%
The number of principal components for PCR is chosen as the number singular values needed to capture at least $99.95\%$ of the spectral energy of $\bY_0$, which yields $k=2$. 
%
In congruence with the theory in Section~\ref{sec:estimation}, we find that the symmetric regressions arrive at the same prediction values from both \HZ~and \VT~approaches. 
%
The asymmetric regressions, on the other hand, produce different \HZ~and \VT~counterfactual trajectories. 
%
We note that the OLS estimate is wildly different from the other estimates and the \HZ~simplex regression puts all mass on the latest pre-intervention time period to become a last observation carried forward (LOCF) estimator. 
%
% ESTIMATION 
\begin{figure} [!t]
	\centering 
	% outcomes equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/basque/outcomes/equal.png}
		\caption{Symmetric regressions.} 
		\label{fig:basque_symmetric} 
	\end{subfigure} 
	\qquad \quad
	% outcomes not equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/basque/outcomes/notequal.png}
		\caption{Asymmetric regressions.} 
		\label{fig:basque_asymmetric} 
	\end{subfigure} 
	\caption{The onset of terrorism is given by the dotted vertical gray line. Basque Country's observed GDP are shown in black. The \HZ~and \VT~counterfactual trajectories are given by solid and dashed-dotted lines, respectively.}
	\label{fig:basque} 
\end{figure}  

% inference 
{\bf Inference.} 
% 
The \HZ~and \VT~in-sample errors were provided in Figure~\ref{fig:basque_res}. 
%
We find that $\bY_0$ has full column rank, i.e., $R = \tr(\bY_0 \bY_0^\dagger) = 15$. 
%
It is no surprise then that the \VT~OLS errors, shown in Figure~\ref{fig:basque_vt_ols_res}, are zero, while the \HZ~OLS errors, shown in Figue~\ref{fig:basque_hz_ols_res}, are nonzero though still small. 
% 
The \HZ~and \VT~PCR in-sample errors are both nonzero, as previously seen in Figures~\ref{fig:basque_hz_pcr_res} and \ref{fig:basque_vt_pcr_res}. 
%
We present the OLS and PCR predictions, along with their corresponding homoskedastic and jackknife confidence intervals, in Figure~\ref{fig:basque_ci}. 
%
We do not apply the HRK estimator as the non-invertibility conditions failed to hold. 

%\clearpage

% CA PROP99
\subsection{California Proposition 99} 

% background 
{\bf Background.} 
%
In this study, we examine the effect of California's Proposition 99, the first modern-time large scale anti-tobacco legislation in the U.S., on its tobacco consumption. 
% 
Per capita cigarette sales across $N = 39$ U.S. states from 1970 to 2000, i.e., $T=31$ years, is collected in this dataset. 
% 
We consider California as our single treated state, which we label as the $N$th state. 
%
The remaining 38 states act as our control states as they neither instituted a tobacco control program nor raised cigarette sales taxes by 50 cents or more. 
%
The introduction of Proposition 99 in 1988 represents the treatment. 
%
Thus, the pre- and post-treatment lengths are $18$ and $13$ years, respectively. 
%
Our primary outcome variable is the per capita cigarette sales. 
%
Our object of interest is the counterfactual time series of sales in the absence of Proposition 99, i.e., $Y_{Nt}(0)$ for $t \in [1988, 2000]$. 
%
Below, we apply the estimators of Section~\ref{sec:estimation} using the following inputs:
%
California's pretreatment sales trajectory, $\by_N \in \Rb^{18}$;  
the control states' pretreatment sales trajectories, $\bY_0 \in \Rb^{38 \times 18}$; 
and the control states' sales during the post-treatment year $t$, $\by_t \in \Rb^{38}$ for $t \in [1988, 2000]$. 

% estimation 
{\bf Estimation.} 
%
Our counterfactual predictions are shown in Figure~\ref{fig:prop99}. 
%
We use the default \texttt{scikit-learn} hyperparameters for the regularized regressions and choose the number of principal components for PCR as the the number singular values needed to capture at least $99.95\%$ of the spectral energy of $\bY_0$, which yields $k=3$. 
% 
Our empirical findings reinforce our results in Section~\ref{sec:estimation} with the symmetric regressions producing the same \HZ~and \VT~predictions and the asymmetric regressions producing different \HZ~and \VT~predictions, even with the same penalty values. 
%
Although the hyperparameters are not tuned, the results across all regressions are qualitatively similar with the exception of \HZ~simplex regression, which again reduces to LOCF. 
%
In fact, the OLS and ridge estimates appear to overlap, as with the lasso and elastic net estimates. 
%
% ESTIMATION
\begin{figure} [!p]
	\centering
	% outcomes equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/equal.png}
		\caption{Symmetric regressions.} 
		\label{fig:prop99_symmetric} 
	\end{subfigure} 
	\qquad \quad
	% outcomes not equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/notequal.png}
		\caption{Asymmetric regressions.} 
		\label{fig:prop99_asymmetric} 
	\end{subfigure} 
	\caption{The passage of Prop 99 is given by the dotted vertical gray line. California's observed sales are shown in black. The \HZ~and \VT~counterfactual trajectories are given by solid and dashed-dotted lines, respectively.}
	\label{fig:prop99} 
\end{figure}  
%
\begin{figure} [!t]
	\centering 
	% OLS hz 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_hz_residuals.png}
		\caption{\HZ~OLS residuals.} 
		\label{fig:prop99_hz_ols_res}
	\end{subfigure} 
	\qquad \quad
	% PCR hz
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_hz_residuals.png}
		\caption{\HZ~PCR residuals.} 
		\label{fig:prop99_hz_pcr_res}
	\end{subfigure} 
	\\
	% OLS vt
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_vt_residuals.png}
		\caption{\VT~OLS residuals.} 
		\label{fig:prop99_vt_ols_res}
	\end{subfigure} 
	\qquad \quad
	% PCR vt
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_vt_residuals.png}
		\caption{\VT~PCR residuals.} 
		\label{fig:prop99_vt_pcr_res}
	\end{subfigure} 
	\caption{
	%
	(Top) The \HZ~OLS and PCR residuals are shown on the left and right, respectively. 
	The vertical line partitions the control states and California. 
	The residuals to the left of the vertical line represent the in-sample errors across control units and post-treatment periods. 
	The residuals to the right of the vertical line represent the treatment effects for California, marked by the red label, over the post-treatment period. 
	(Bottom) The \VT~OLS and PCR residuals are shown on the left and right, respectively. 
	The vertical line partitions the pre- and post-treatment periods with the latter labeled in red. 
	The residuals to the left of the vertical line represent California's in-sample errors over the pretreatment period.
	The residuals to the right display the same treatment effects over time for California as shown in the top figures.
	}
	\label{fig:prop99_res} 
\end{figure}  

 % inference
{\bf Inference.} 
%
We display the \HZ~and \VT~residuals in Figure~\ref{fig:prop99_res}.
% 
We find that $\bY_0$ has rank $R = \tr(\bY_0 \bY_0^\dagger) = 17$. 
%
The \VT~OLS in-sample errors are zero while the \HZ~OLS in-sample errors are distributed between $[-20, 20]$. 
% 
The \HZ~and \VT~PCR in-sample errors are distributed between $[-35, 35]$ and $[-5, 5]$, respectively. 
% 
For OLS and PCR, we apply the homoskedastic and jackknife intervals since the conditions for the HRK interval are not satisfied. 
%
The resulting intervals are shown in Figure~\ref{fig:prop99_ci.1} and \ref{fig:prop99_ci.2}. 
%
As expected, the \VT~OLS confidence intervals are degenerate. %collapse around its predictions. 
%
In contrast, the \HZ~and mixed confidence intervals expand over time. 
%
The jackknife intervals are generally larger than the homoskedastic intervals, which is expected given that the jackknife is conservative. 
%
Further, the \VT~PCR confidence intervals are tightly centered around the prediction values but are nontrivial. 
%
In all other aspects, the PCR confidence intervals are similar to that of OLS. 
%

% CONFIDENCE INTERVALS OLS
\begin{figure} [!p]
	\centering
	% OLS HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_hz_homoskedastic.png}
		\caption{\HZ~OLS homoskedastic.} 
	\end{subfigure} 
	% OLS VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_vt_homoskedastic.png}
		\caption{\VT~OLS homoskedastic.} 
	\end{subfigure} 
	% OLS HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_hz-vt_homoskedastic.png}
		\caption{Mixed OLS homoskedastic.} 
	\end{subfigure} 	
	% OLS HZ-jack
	\\
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_hz_jackknife.png}
		\caption{\HZ~OLS jackknife.} 
	\end{subfigure} 
	% OLS VT-jack
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_vt_jackknife.png}
		\caption{\VT~OLS jackknife.} 
	\end{subfigure} 
	% OLS HZ-VT-jack
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/ols_hz-vt_jackknife.png}
		\caption{Mixed OLS jackknife.} 
	\end{subfigure} 
	\caption{
	OLS predictions and confidence intervals. 
	We index rows by the covariance estimator, e.g., jackknife, and the columns by the type of confidence interval, e.g., \HZ.   
}
	\label{fig:prop99_ci.1} 
\end{figure} 

% CONFIDENCE INTERVALS PCR 
\begin{figure} [!p]
	\centering 
	% PCR HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_hz_homoskedastic.png}
		\caption{\HZ~PCR homoskedastic.} 
	\end{subfigure} 
	% PCR VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_vt_homoskedastic.png}
		\caption{\VT~PCR homoskedastic.} 
	\end{subfigure} 
	% PCR HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_hz-vt_homoskedastic.png}
		\caption{Mixed PCR homoskedastic.} 
	\end{subfigure} 	
	\\
	% PCR HZ-jack
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_hz_jackknife.png}
		\caption{\HZ~PCR jackknife.} 
	\end{subfigure} 
	% PCR VT-jack
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_vt_jackknife.png}
		\caption{\VT~PCR jackknife.} 
	\end{subfigure} 
	% PCR HZ-VT-jack
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/outcomes/pcr_hz-vt_jackknife.png}
		\caption{Mixed PCR jackknife.} 
	\end{subfigure} 	
	\caption{
	PCR predictions and confidence intervals. 
	We index rows by the covariance estimator, e.g., jackknife, and the columns by the type of confidence interval, e.g., \HZ. 
	}
	\label{fig:prop99_ci.2} 
\end{figure}  


\clearpage 

% WEST GERMANY 
\subsection{West Germany Reunification} \label{sec:west_germany} 

% background 
{\bf Background.} 
%
We examine the economic impact of the 1990 German reunification in West Germany. 
%
This dataset comprises of $N=17$ countries and their recorded per capita GDPs from 1960-2003, i.e., $T=44$ years. 
%
West Germany represents our single treated country $N$ and the remaining 16 countries serve as our control countries. 
%
The reunification in 1990 represents the treatment, which set the pre- and post-intervention lengths as $30$ and $14$ years, respectively. 
%
The per capita GDP is the primary outcome variable and our goal is to estimate West Germany's counterfactual GDP trajectory in the absence of reunification, i.e., $Y_{Nt}(0)$ for $t \in [1990, 2003]$. 
%
We apply the estimators of Section~\ref{sec:estimation} using the following inputs:
%
West Germany's pre-intervention GDP trajectory, $\by_N \in \Rb^{30}$;  
the control countries' pre-intervention GDP trajectories, $\bY_0 \in \Rb^{16 \times 30}$; 
and the control countries' GDPs during the post-intervention year $t$, $\by_t \in \Rb^{16}$ for $t \in [1990, 2003]$. 

% estimation 
{\bf Estimation.} 
%
We present the counterfactual estimates in Figure~\ref{fig:germany} using the default \texttt{scikit-learn} hyperparameters for the regularized estimators and choosing the number of principal components for PCR as the the number singular values needed to capture at least $99.95\%$ of the spectral energy of $\bY_0$, which yields $k=3$. 
% 
Our empirical findings provide further evidence of the formal statements in Section~\ref{sec:estimation}. 
%
Much like the California Proposition 99 study, we notice that the results across all regressions are qualitatively similar with the exception of \HZ~simplex regression, which once more reduces to a LOCF estimator. 
% 
In particular, we observe that OLS and ridge overlap again, similar to lasso and elastic net. 

% ESTIMATION
\begin{figure} [!p]
	\centering
	% outcomes equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/equal.png}
		\caption{Symmetric regressions.} 
		\label{fig:germany_symmetric} 
	\end{subfigure} 
	\qquad \quad
	% outcomes not equal 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/notequal.png}
		\caption{Asymmetric regressions.} 
		\label{fig:germany_asymmetric} 
	\end{subfigure} 
	\caption{%West Germany Reunification. 
	The reunification is given by the dotted vertical gray line. West Germany's observed GDP is shown in black. The \HZ~and \VT~counterfactual trajectories are given by solid and dashed-dotted lines, respectively.}
	\label{fig:germany} 
\end{figure} 

% inference
{\bf Inference.} 
%
We display the \HZ~and \VT~OLS and PCR residuals in Figure~\ref{fig:germany_res}.
% 
We find that $\bY_0$ has full row rank with $R = \tr(\bY_0 \bY_0^\dagger) = 16$. 
%
Thus, the \HZ~OLS in-sample errors are zero while the \VT~OLS in-sample errors are small but nonzero. 
% 
The \HZ~PCR in-sample errors are roughly distributed between $[-4000, 4000]$ and the \VT~PCR in-sample errors are much smaller in magnitude. 
% 
For OLS, we apply the \HZ, \VT, and Mixed homoskedastic and jackknife variance estimators since the conditions for the HRK variance estimator are not satisfied. 
%
The resulting intervals are shown in Figures~\ref{fig:germany_hz_homo}--\ref{fig:germany_hz-vt_jack}. 
%
For PCR, we apply all variance estimators, including HRK. 
%
The HRK based intervals are provided in Figure~\ref{fig:germany_ci.2}, while the remaining were previously displayed in Figures~\ref{fig:germany_hz_homo.pcr}--\ref{fig:germany_hz-vt_jack.pcr}.
%The resulting confidence intervals are shown in Figure~\ref{fig:germany_ci.1} and \ref{fig:germany_ci.2}. 
%
To no surprise, the OLS \HZ~confidence intervals are degenerate. 
%
The OLS \VT~and mixed confidence intervals, on the other hand, expand over time. 
%
In general, the jackknife intervals engulf the homoskedastic intervals. 
%
For PCR, we observe that the \HZ~confidence intervals are tightly centered around the prediction values but the \VT~confidence intervals also increase over time. 

% RESIDUALS
\begin{figure} [!p]
	\centering 
	% OLS hz 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/ols_hz_residuals.png}
		\caption{\HZ~OLS residuals.} 
		\label{fig:germany_hz_ols_res}
	\end{subfigure} 
	\qquad \quad
	% PCR hz
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/pcr_hz_residuals.png}
		\caption{\HZ~PCR residuals.} 
		\label{fig:germany_hz_pcr_res}
	\end{subfigure} 
	\\
	% OLS vt
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/ols_vt_residuals.png}
		\caption{\VT~OLS residuals.} 
		\label{fig:germany_vt_ols_res}
	\end{subfigure} 
	\qquad \quad
	% PCR vt
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/pcr_vt_residuals.png}
		\caption{\VT~PCR residuals.} 
		\label{fig:germany_vt_pcr_res}
	\end{subfigure} 
	\caption{
	%
	(Top) The \HZ~OLS and PCR residuals are shown on the left and right, respectively. 
	The vertical line partitions the control countries and West Germany. 
	The residuals to the left of the vertical line represent the in-sample errors across control units and post-treatment periods. 
	The residuals to the right of the vertical line represent the treatment effects for West Germany, marked by the red label, over the post-treatment period. 
	(Bottom) The \VT~OLS and PCR residuals are shown on the left and right, respectively. 
	The vertical line partitions the pre- and post-treatment periods with the latter labeled in red. 
	The residuals to the left of the vertical line represent West Germany's in-sample errors over the pretreatment period.
	The residuals to the right display the same treatment effects over time for West Germany as shown in the top figures.
	}
	\label{fig:germany_res} 
\end{figure}   

% CONFIDENCE INTERVALS PCR
\begin{figure} [!t]
	\centering 
	% PCR HZ-hrk
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/pcr_hz_HRK.png}
		\caption{\HZ~PCR HRK.} 
	\end{subfigure} 
	% PCR VT-hrk
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/pcr_vt_HRK.png}
		\caption{\VT~PCR HRK.} 
	\end{subfigure} 
	% PCR HZ-VT-hrk
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany/outcomes/pcr_hz-vt_HRK.png}
		\caption{Mixed PCR HRK.} 
	\end{subfigure} 	
	\caption{PCR predictions with confidence intervals. 
	The intervals are constructed from the HRK covariance estimator. 
	We index %rows by the covariance estimator, e.g., jackknife, and the 
	columns by the type of confidence interval, e.g., \HZ. 
	}
	\label{fig:germany_ci.2} 
\end{figure}  

\subsection{Common Themes} 
%
We discuss a few common themes from our empirical illustrations. 
%
First, with respect to estimation, our findings support our classification results in Section~\ref{sec:estimation}. 
%
Notably, we observe that the simplex constraint induces the greatest asymmetry between the \HZ~and \VT~predictions. 
%
In every study, including the Basque study presented in the main body, \HZ~simplex regression reduces to the LOCF predictor. 
%
This suggests that that the simplex constraint imposes a strong systematic structure on the underlying DGP. 
%
Finally, with respect to inference, our results provide further evidence in support of the mixed interval by showcasing its robustness relative to the \HZ~and \VT~intervals. 

% include intercepts for estimation 
%\newpage


==> content/inference_2.tex <==
\section{Large-Sample Inference} \label{sec:inference} 
%
\smallskip 
\begin{tcolorbox}[colback=gray!10!white,colframe=black!75!black]
	\begin{center}
	{
		{\bf Q2:} ``Why do \HZ~and \VT~confidence intervals differ \\ when their estimates agree?'' 
	} 
	\end{center} 
\end{tcolorbox}
%
\smallskip 
%
To answer Q2, we study the inferential properties of the counterfactual prediction. 
%the $(N,T)$th counterfactual prediction. %\HZ~and \VT~regressions. 
%
Formal discussions for classical inference require an explicit postulation of the repeated sampling procedure.  
%
Broadly speaking, there are two schools of thought. 
%
The first is model-based, which makes assumptions about the distribution of the potential outcomes. 
%
The second is design-based, which makes assumptions about the selection of treated units and time periods.  
% 
This article takes a model-based route that is similar in parts to the recent works of \cite{li2020}, \cite{cattaneo}, and \cite{sc_lasso1, sc_t_test} from the synthetic controls literature. 
%
We offer connections to design-based approaches at the section's end. 
%

For ease of exposition, we focus on OLS and its minimum $\ell_2$-norm solutions, i.e., $\bhalpha = \bY_0^\dagger \by_T$ and $\bhbeta = (\bY'_0)^\dagger \by_N$. 
%
As such, we define $\hY_{NT}(0) = \hY^\hz_{NT}(0) = \hY^\vt_{NT}(0)$, which is justified under Theorem~\ref{thm:equivalent}. 
%
Our results immediately extend to PCR by replacing $\bY_0$ with $\bY_0^{(k)}$, as defined in \eqref{eq:rank_k}, for any $k < R$. 
%
%By Theorem~\ref{thm:equivalent}, we define $\hY_{NT}(0) = \hY^\hz_{NT}(0) = \hY^\vt_{NT}(0)$. 
%
To improve readability, we present several results informally and provide their precise versions in Appendix~\ref{sec:appendix_inference}. 

%\begin{center}
%	{
%		{\bf Q2:} ``Why do \HZ~and \VT~confidence intervals differ when their estimates agree?'' 
%	} 
%\end{center} 
%Towards answering Q2, we study the asymptotic properties of \HZ~and \VT~approaches. 
%%
%In this pursuit, we require probabilistic generative modeling assumptions. 
%%
%This section subscribes to concepts from the standard regression framework, which we believe is a natural starting point to extract valuable insights. 
%%
%For ease of exposition, we focus on OLS and its minimum $\ell_2$-norm solutions, $\bhalpha = \bY_0^\dagger \by_T$ and $\bhbeta = (\bY'_0)^\dagger \by_N$. 
%%
%Notably, our results immediately extend to PCR by replacing $\bY_0$ with $\bY_0^{(k)}$, as defined in \eqref{eq:rank_k}, for any $k < R$. 
%%
%We state some of our results informally to improve readability and provide the precise forms in Appendix~\ref{sec:appendix_inference}. 

% ASYMPTOTIC UNDER DISTINCT
\subsection{Inference under Distinct Generative Models}
\label{sec:isolated} 
%
Within the model-based framework, we consider a regression model. 
%
This postulation is not always plausible but it is useful to dissect its implications. 
%
In this vein, we now study the properties of $\hY_{NT}(0)$ under distinct \HZ~and \VT~regressions models. 
%it is a natural and humble starting point to extract valuable insights. 
%Although this postulation is not always plausible, %it is useful to consider its implications. 
%it is a natural and humble starting point to extract valuable insights. 
%In this vein, we now study the two approaches under their respective regressions models. 


% generative models
\subsubsection{Generative Models} \label{sec:isolated_assump} 
%
Mirroring the definitions of $(\by_N, \by_T)$, we denote $\bvarepsilon_T = [\varepsilon_{iT}: i \le N_0]$ as the errors associated with the control units during treated period and $\bvarepsilon_N = [\varepsilon_{Nt}: t \le T_0]$ as the errors associated with the treated unit during the pretreatment period. 
%
\begin{assumption} [\HZ~generative model] \label{assump:hz} 
%
Conditional on $(\by_N, \bY_0)$, 
%\hfill 
%
\begin{itemize}
	\item[(i)] there exists an $\balpha^* \in \Rb^{T_0}$ such that 
	$Y_{iT} = \sum_{t \le T_0} \alpha^*_t Y_{it} + \varepsilon_{iT}$ for $i \le N$. 
	%(a) $\by_T = \bY_0 \balpha^* + \bvarepsilon_T$ and (b) $\Ex[Y_{NT}(0) | \by_N] = \langle \by_N, \balpha^* \rangle$. 
	
	\item[(ii)] $\varepsilon_{iT}$ are mean zero for $i \le N$. 
	%$\Ex[\bvarepsilon_T | \bY_0] = \bzero$. 
 
	\item[(iii)] $\varepsilon_{iT}$ are independent over $i \le N$. 
	%outcomes are sampled independently across units. 
	
	\item[(iv)] one of the following holds: 
	\begin{enumerate} 
		\item[(a)] $\balpha^* \in \emph{rowspan}(\bY_0)$
		\item[(b)] $\by_N \in \emph{rowspan}(\bY_0)$. 
	\end{enumerate} 
\end{itemize} 
\end{assumption} 
%\begin{itemize}
%	\item[(i)] {\em Outcome model:} 
%	$Y_{iT} = \sum_{t \le T_0} \alpha^*_t Y_{it} + \varepsilon_{iT}$ for $i \le N$. 
%	%(a) $\by_T = \bY_0 \balpha^* + \bvarepsilon_T$ and (b) $\Ex[Y_{NT}(0) | \by_N] = \langle \by_N, \balpha^* \rangle$. 
%	
%	\item[(ii)] {\em Strict exogeneity:} $\Ex[\varepsilon_{iT} | \bY_0] = 0$ for $i \le N$. 
%	%$\Ex[\bvarepsilon_T | \bY_0] = \bzero$. 
% 
%	\item[(iii)] {\em Independence:} $\bvarepsilon_T$ is independent over $i$ conditional on $\bY_0$. 
%	%outcomes are sampled independently across units. 
%	
%	\item[(iv)] {\em Subspace inclusion:} denote $\balpha^* = [\alpha^*_t: t \le T_0]$ and let one of the following hold: 
%	\begin{enumerate} 
%		\item[(a)] $\balpha^* \in \emph{rowspan}(\bY_0)$
%		\item[(b)] $\by_N \in \emph{rowspan}(\bY_0)$. 
%	\end{enumerate} 
%\end{itemize} 
%\end{assumption} 

%\pagebreak 
\begin{assumption} [\VT~generative model] \label{assump:vt} 
%
Conditional on $(\by_T, \bY_0)$, 
%\hfill
%
\begin{itemize}
%
	\item[(i)] there exists a $\bbeta^* \in \Rb^{N_0}$ such that $Y_{Nt} = \sum_{i \le N_0} \beta^*_i Y_{it} + \varepsilon_{Nt}$ for $t \le T$. 
	%(a) $\by_N = \bY'_0 \bbeta^* + \bvarepsilon_N$ and (b) $\Ex[Y_{NT}(0) | \by_T] = \langle \by_T, \bbeta^* \rangle$. 
		
	\item[(ii)] $\varepsilon_{Nt}$ are mean zero for $t \le T$. 
	%$\Ex[\bvarepsilon_N | \bY_0] = \bzero$. 
	
	\item[(iii)] $\varepsilon_{Nt}$ are independent over $t \le T$. 
	%outcomes are sampled independently across time.  
	
	\item[(iv)] one of the following holds: 
	\begin{enumerate} 
		\item[(a)] $\bbeta^* \in \emph{rowspan}(\bY'_0)$
		\item[(b)] $\by_T \in \emph{rowspan}(\bY'_0)$.
	\end{enumerate} 
	%(a) $\bbeta^* \in \emph{colspan}(\bY_0)$ or (b) $\by_T \in \emph{colspan}(\bY_0)$ . 
%
\end{itemize} 
%\begin{itemize}
%%
%	\item[(i)] {\em Outcome model:} $Y_{Nt} = \sum_{i \le N_0} \beta^*_i Y_{it} + \varepsilon_{Nt}$ for $t \le T$. 
%	%(a) $\by_N = \bY'_0 \bbeta^* + \bvarepsilon_N$ and (b) $\Ex[Y_{NT}(0) | \by_T] = \langle \by_T, \bbeta^* \rangle$. 
%		
%	\item[(ii)] {\em Strict exogeneity:} $\Ex[\varepsilon_{Nt} | \bY_0] = 0$ for $t \le T$. 
%	%$\Ex[\bvarepsilon_N | \bY_0] = \bzero$. 
%	
%	\item[(iii)] {\em Independence:} $\bvarepsilon_N$ is independent over $t$ conditional on $\bY_0$. 
%	%outcomes are sampled independently across time.  
%	
%	\item[(iv)] {\em Subspace inclusion:} denote $\bbeta^* = [\beta^*_i: i \le N_0]$ and let one of the following hold: 
%	\begin{enumerate} 
%		\item[(a)] $\bbeta^* \in \emph{rowspan}(\bY'_0)$
%		\item[(b)] $\by_T \in \emph{rowspan}(\bY'_0)$.
%	\end{enumerate} 
%	%(a) $\bbeta^* \in \emph{colspan}(\bY_0)$ or (b) $\by_T \in \emph{colspan}(\bY_0)$ . 
%%
%\end{itemize} 
\end{assumption} 
%
We interpret Assumptions~\ref{assump:hz} and \ref{assump:vt} through a panel data lens. 

% outcome model 
\smallskip 
\noindent 
{\bf (i) Outcome model.} 
%
Assumption~\ref{assump:hz} (i) explicitly models time series patterns as the source of randomness in the \HZ~framework. 
%
Assumption~\ref{assump:vt} (i) explicitly models cross-sectional patterns as the source of randomness in the \VT~framework. 
%
Thus, the statistical uncertainty of $\hY_{NT}(0)$ under the \HZ~model is 
%Put differently, the \HZ~model postulates that the statistical uncertainty of the counterfactual prediction is 
governed by the construction of the regression model $\bhalpha$ from the control units' outcomes $(\by_T, \bY_0)$---this captures the in-sample uncertainty. 
% 
An analogous statement holds for the \VT~model with respect to $\bhbeta$ and the pretreatment outcomes $(\by_N, \bY_0)$. 
%
Each model posits that their correlation pattern of interest obeys a linear relationship. 

%The construction begins by noting that the statistical uncertainty of the SC prediction is governed by two distinct sources of randomness: one coming from the construction of the (likely misspecified) SC weights in the pretreatment period

% strict exogeneity 
\smallskip 
\noindent 
{\bf (ii) Strict exogeneity.} 
%
Condition (ii) implies that the errors have zero mean and the regressors (e.g., lagged outcomes) are uncorrelated with the errors. 

% independence
\smallskip 
\noindent 
{\bf (iii) Independence.} 
%
Assumption~\ref{assump:hz} (iii) allows time correlated errors in the \HZ~framework. 
%
Assumption~\ref{assump:vt} (iii) allows unit correlated errors in the \VT~framework. 
%
%We leave a proper study under correlated errors, as in the works above, for future research. 

% subspace inclusion
\smallskip 
\noindent 
{\bf (iv) Subspace inclusion.} 
%
We justify condition (iv). 
%
Consider the \HZ~perspective.
%
Let $\bH^v = \bV \bV'$ and $\bH^v_\perp = \bI - \bV \bV'$. 
%
Since $\bhalpha = \bH^v \bhalpha$, we obtain 
%
\begin{align}
	\hY_{NT}(0) - \Ex[Y_{NT}(0) | \by_T, \bY_0]
	%&= \langle \by_N, \bhalpha - \balpha^* \rangle 
	= \langle \by_N, \bhalpha - \bH^v \balpha^* \rangle - \underbrace{\langle \bH^v_\perp \by_N, \bH^v_\perp \balpha^* \rangle}_{\text{excess}}. \label{eq:intuition} 
\end{align} 
%
From \eqref{eq:intuition}, we see that the excess prediction error vanishes if Assumption~\ref{assump:hz} (iv) holds. 
%
Although this condition may be cosmetically unfamiliar, it is actually implied by the canonical full rank assumption, i.e., $\text{rank}(\bY_0) = T_0$ and hence $\text{rowspan}(\bY_0) = \Rb^{T_0}$. 
%
Accordingly, $\bH^v_\perp \balpha^* = \bzero$ and $\bH^v_\perp \by_N = \bzero$ necessarily. 
%
From this perspective, Assumption~\ref{assump:hz} (iv) generalizes the full column rank assumption to rank deficient scenarios. 
%generalizes the full column rank assumption to handle scenarios where $\bY_0$ is rank deficient. 
%
This is our focus as we do not impose restrictions on the relative sizes of $N$ and $T$. 

%Though cosmetically different,  
%condition (iv) is implicitly assumed in the standard OLS framework. 
%%
%Consider \HZ~regression. 
%%
%Typically, it is assumed that $R = \text{rank}(\bY_0) = T_0$, i.e., $\text{rowspan}(\bY_0) = \Rb^{T_0}$. 
%%
%Accordingly, $\balpha^* \in \text{rowspan}(\bY_0)$ and $\by_N \in \text{rowspan}(\bY_0)$, so (iv) immediately holds. 
%%
%From this perspective, Assumption~\ref{assump:hz} (iv) is a generalization of the canonical full column rank assumption to handle scenarios where $\bY_0$ is rank deficient. 
%%
%This is our focus as we do not assume the sizes of $N$ and $T$. 
%

To internalize the general setting, we zoom in on (iv.a) and consider the extreme scenario where $\balpha^* = \bH^v_\perp \balpha^*$, i.e., $\balpha^*$ is entirely embedded within the nullspace of $\bY_0$. 
%
There, $\bhalpha$ becomes a meaningless predictive model.  
%
By contrast, if (iv.a) holds, then $\bhalpha$ can recover $\balpha^*$ and generalize to the $(N,T)$th point.  
%
We apply a similar thought experiment to (iv.b) by considering $\by_N = \bH^v_\perp \by_N$. 
%
Again, $\bhalpha$ is unlikely to predict well on $\by_N$ since $\bhalpha$ is trained on in-sample data that are highly dissimilar (orthogonal) to $\by_N$. 
%
By contrast, if (iv.b) holds, then $\by_N$ resembles the in-sample data and can generalize to the $(N,T)$th point. %, provided the in-sample error, $\by_T - \bY_0 \bhalpha$, is small.
%
In fact, (iv.b) can be rewritten as the existence of a vector $\bb$ such that $\by_N = \bY_0' \bb$. 
%
This is precisely Assumption~\ref{assump:vt} (i) if $\bvarepsilon_N = \bzero$.  
%
Hence, Assumption~\ref{assump:hz} (iv.b) assumes a deterministic \VT~outcome model. 
%
Since the same arguments apply for \VT~regression, this suggests \HZ~regression implicitly relies on cross-sectional patterns and \VT~regression implicitly relies on time series patterns. 

% summary 
\smallskip 
\noindent 
{\bf Summary.} 
%
Assumptions~\ref{assump:hz} and \ref{assump:vt} describe fundamentally different DGPs that cannot simultaneously hold for the same data. 
% 
Therefore, it is arduous to compare the two approaches beyond point estimation. 

% remark
\begin{remark}
%
For expositional convenience, we assume correct specification of the outcome model, as in \cite{li2020}, to explain the panel data intuition and main theoretical results in a simple and transparent fashion. 
%
Alternatively, we can interpret Assumptions~\ref{assump:hz} and \ref{assump:vt} as a linear prediction model that is detached from structural meanings a la \cite{cattaneo} and \cite{sc_lasso1, sc_t_test}. 
%
This redefines $\balpha^* = \argmin \Ex[ \| \by_T - \bY_0 \balpha \|_2^2 | \bY_0]$ as the best linear approximation of $\by_T$ based on $\bY_0$, conditional on $\bY_0$; 
%
$\bbeta^*$ is redefined analogously.  
%
Such models can be justified via factor models and vector autoregressive models \citep{sc_t_test}.  
%
\end{remark} 

% results 
\subsubsection{Asymptotic Properties} 
%
Equipped with our assumptions, we are ready to formally answer Q2. %present the \HZ~and \VT~asymptotic properties. 
%%
We denote the \HZ~and \VT~causal estimands as $\mu_0^\hz = \Ex[Y_{NT}(0) | \by_N, \bY_0]$ and $\mu_0^\vt = \Ex[Y_{NT}(0) | \by_T, \bY_0]$, respectively.  
%
We denote the error covariance matrices as  
% 
\begin{align}
	&\bSigma_T = \Cov(\bvarepsilon_T | \bY_0) = \text{diag}(\sigma^2_{1T}, \dots, \sigma^2_{N_0 T})
	\\ 
	&\bSigma_N = \Cov(\bvarepsilon_N | \bY_0) = \text{diag}(\sigma^2_{N1}, \dots, \sigma^2_{N T_0}).
\end{align} 
%
\begin{theorem} \label{thm:inference} 
%
Let Assumption~\ref{assump:hz} hold. 
%
%Conditional on $(\by_N, \bY_0)$ and 
Under suitable moment conditions, 
%
\begin{align}
	& \frac{\hY_{NT}(0) - \mu_0^\ehz}{ \sqrt{v_0^\ehz}} \xrightarrow{d} \mathcal{N}(0,1), 
\end{align} 
%
where $v_0^\ehz = \bhbeta' \bSigma_T \bhbeta$. 
%
Let Assumption~\ref{assump:vt} hold. 
%
%Conditioned on $(\by_T, \bY_0)$ and 
Under suitable moment conditions, 
%
\begin{align}
	\frac{\hY_{NT}(0) - \mu_0^\evt}{ \sqrt{v^\evt_0}} \xrightarrow{d} \mathcal{N}(0,1), 
\end{align} 
%
where $v^\evt_0 = \bhalpha' \bSigma_N \bhalpha$.  
\end{theorem} 
%
Theorem~\ref{thm:inference} states that the asymptotic variance of $\hY_{NT}(0)$ is controlled by time series patterns under the \HZ~model and cross-sectional patterns under the \VT~model.  
%
This difference is expected given that the two models measure uncertainty with respect to a different parameter and over a different probability measure. 
% 
We scrutinize the consequences of this asymmetry next. 

%%As expected, Theorem~\ref{thm:inference} states that the \HZ~and \VT~asymptotic variances 
%Theorem~\ref{thm:inference} states that the \HZ~and \VT~asymptotic variances are controlled by time series and cross-sectional patterns, respectively. 
%statistical uncertainties of the \HZ~and \VT~predictions are purely governed by time series and cross-sectional patterns, respectively. 
%\HZ~and \VT~asymptotic variances are controlled by time series and cross-sectional patterns, respectively. 

% CONFIDENCE INTERVALS
\subsubsection{Confidence Intervals} \label{sec:ci.1} 
%
Theorem~\ref{thm:inference} motivates separate \HZ~and \VT~confidence intervals: for $\theta \in (0,1)$, 
%
\begin{align} 
	&\text{(\HZ~confidence interval)} \quad \mu_0^\hz \in \left[ \hY_{NT}(0) ~\pm~ z_{\frac \theta 2} \sqrt{\hv^\hz_0} \right] 
	\\
	&\text{(\VT~confidence interval)} \quad \mu_0^\vt \in \left[ \hY_{NT}(0) ~\pm~ z_{\frac \theta 2} \sqrt{\hv^\vt_0} \right], \label{eq:ci.0} 
\end{align}
%
where 
$z_{\frac \theta 2}$ is the upper $\theta/2$ quantile of $\mathcal{N}(0,1)$, 
and 
$(\hv^\hz_0, \hv^\vt_0)$ are the estimators of $(v^\hz_0, v^\vt_0)$. 
%
We construct 
%
\begin{align}
	\hv^\hz_0 = \bhbeta' \bhSigma_T \bhbeta 
	\quad \text{and} \quad 
	\hv^\vt_0 = \bhalpha' \bhSigma_N \bhalpha, 
	\label{eq:hz_vt_specific_estimators}
\end{align}  
%
where $(\bhSigma_T, \bhSigma_N)$ are the estimators of $(\bSigma_T, \bSigma_N)$. 
%
We precisely define these estimators under homoskedastic and heteroskedastic errors below. 
%
To reduce ambiguity, we index $\hv_0^\hz$ and $\hv_0^\vt$ by the covariance estimator. 
%
We also denote $\bH^u = \bU \bU'$ and $\bH^u_\perp = \bI - \bH^u$. 
%  $\bH^v = \bV \bV'$, and $\bH^v_\perp = \bI - \bH^v$. 
%
With this notation, the \HZ~and \VT~in-sample prediction errors can be written as $\bH^u_\perp \by_T = \by_T - \bY_0 \bhalpha$ 
and $\bH^v_\perp \by_N = \by_N - \bY'_0 \bhbeta$, respectively.

% Homoskedasticity
\smallskip 
\noindent 
{\bf Homoskedastic errors.} 
%
Consider $\bSigma_T = \sigma^2_T \bI$ and $\bSigma_N = \sigma^2_N \bI$. 
%
We design
%
\begin{align}
	&\bhSigma_T^\homo = \hsigma^2_T \bI ~~\text{with}~~ \hsigma^2_T = (N_0-R)^{-1} \| \bH^u_\perp \by_T \|_2^2, 	\label{eq:hz.var.1} 
	\\
	&\bhSigma_N^\homo = \hsigma^2_N  \bI ~~\text{with}~~ \hsigma^2_N = (T_0-R)^{-1} \| \bH^v_\perp \by_N \|_2^2, \label{eq:vt.var.1} 
\end{align}  
%
where %$R = \text{rank}(\bY_0) = \tr(\bH^u) = \tr(\bH^v)$. 
$R = \text{rank}(\bY_0)$, which can be computed as $R = \tr(\bH^u) = \tr(\bH^v)$. 

% lemma 
\begin{lemma} \label{lemma:inference.1} 
%
%Consider homoskedastic errors.  
%
Under Assumption~\ref{assump:hz}, 
$\Ex[\bhSigma_T^\ehomo | \bY_0] =  \bSigma_T$; thus, 
$\Ex[ \hv^{\ehz, \ehomo}_0 | \by_N, \bY_0] = v^\ehz_0$. 
%
Under Assumption~\ref{assump:vt},  
$\Ex[ \bhSigma_N^\ehomo | \bY_0] = \bSigma_N$; thus, $\Ex[ \hv^{\evt, \ehomo}_0 | \by_T, \bY_0] = v^\evt_0$. 
  
\end{lemma} 
%
Lemma~\ref{lemma:inference.1} is a well known result within the OLS literature, albeit it is typically formalized under the stricter full column rank assumption. 

% Heteroskedasticity
\smallskip 
\noindent 
{\bf Heteroskedastic errors.}  
%
We adopt two strategies for the heteroskedastic setting. 

% Jackknife 
\smallskip 
\noindent 
{\em I: Jackknife.} 
%
The first estimator is based on the jackknife. 
%
Traditionally, the jackknife estimates the covariance of the regression models $(\bhalpha, \bhbeta)$. 
% 
By analyzing said estimates, we can then derive the following: 
%
\begin{align}
	\bhSigma_T^\jack &= 
	\text{diag}\left( \left[ \bH^u_\perp \circ  \bH^u_\perp \circ \bI \right]^\dagger \left[  \bH^u_\perp \by_T \circ  \bH^u_\perp \by_T \right] \right) \label{eq:hz.var.2} 
	\\ 
	\bhSigma_N^\jack &= 
	\text{diag}\left( \left[ \bH^v_\perp \circ  \bH^v_\perp \circ \bI  \right]^\dagger \left[ \bH^v_\perp \by_N \circ \bH^v_\perp \by_N \right]\right).  \label{eq:vt.var.2} 
\end{align} 
%
\begin{lemma} \label{lemma:inference.2} 
%
%Consider heteroskedastic errors. 
%
Let Assumption~\ref{assump:hz} hold. 
%
If $(\bH^u_\perp \circ  \bH^u_\perp \circ \bI)$ is nonsingular, then $\Ex[\bhSigma^\ejack_T | \bY_0] \succeq \bSigma_T$; thus, $\Ex[ \hv^{\ehz, \ejack}_0 | \by_N, \bY_0] \ge v^\ehz_0$. 
%
Let Assumption~\ref{assump:vt} hold. 
%
If $(\bH^v_\perp \circ  \bH^v_\perp \circ \bI)$ is nonsingular, then $\Ex[\bhSigma^\ejack_N | \bY_0] \succeq \bSigma_N$; thus, $\Ex[ \hv^{\evt, \ejack}_0 | \by_T, \bY_0] \ge v^\evt_0$. 
\end{lemma} 
%
Lemma~\ref{lemma:inference.2} establishes that the jackknife is conservative, provided $(\bH^u_\perp \circ  \bH^u_\perp \circ \bI)$ and $(\bH^v_\perp \circ  \bH^v_\perp \circ \bI)$ are nonsingular. 
%
Strictly speaking, the jackknife is well defined if these quantities are singular, as seen through the pseudoinverse in \eqref{eq:hz.var.2} and \eqref{eq:vt.var.2}. 
%
Lemma~\ref{lemma:inference.2} considers the nonsingular case for simplicity.  
%
We remark that $\max_\ell H^u_{\ell \ell} < 1$ and $\max_\ell H^v_{\ell \ell} < 1$ are sufficient conditions for invertibility. 
%

% Hartley
\smallskip 
\noindent 
{\em II: HRK-estimator.} 
%
Next, we consider the covariance estimator proposed by \cite{variance}. 
%
We index this estimator by the authors, Hartley-Rao-Kiefer. 
%
\begin{align}
	\bhSigma_T^\hrk &=  \text{diag}\left( \left[ \bH^u_\perp \circ  \bH^u_\perp \right]^{-1} \left[  \bH^u_\perp \by_T \circ  \bH^u_\perp \by_T \right] \right)  \label{eq:hz.var.3} 
	\\ 
	\bhSigma_N^\hrk &= \text{diag}\left( \left[ \bH^v_\perp \circ \bH^v_\perp \right]^{-1} \left[ \bH^v_\perp \by_N \circ \bH^v_\perp \by_N \right] \right). \label{eq:vt.var.3} 
\end{align} 
% 
\begin{lemma} \label{lemma:inference.3} 
%
%Consider heteroskedastic errors. 
%
Let Assumption~\ref{assump:hz} hold. 
%
If $(\bH^u_\perp \circ  \bH^u_\perp)$ is nonsingular, then $\Ex[\bhSigma^\ehrk_T | \bY_0] = \bSigma_T$; thus, $\Ex[ \hv^{\ehz, \ehrk}_0 | \by_N, \bY_0] = v^\ehz_0$. 
%
Let Assumption~\ref{assump:vt} hold. 
%
If $(\bH^v_\perp \circ  \bH^v_\perp)$ is nonsingular, then $\Ex[\bhSigma^\ehrk_N | \bY_0] = \bSigma_N$; thus, $\Ex[ \hv^{\evt, \ehrk}_0 | \by_T, \bY_0] = v^\evt_0$. 
%
\end{lemma} 
%
Lemma~\ref{lemma:inference.3} establishes that the HRK estimator is unbiased, provided $(\bH^u_\perp \circ  \bH^u_\perp)$ and $(\bH^v_\perp \circ \bH^v_\perp)$ are invertible. 
%
For the former quantity, $\max_\ell H^u_{\ell \ell} < 1/2$ is a sufficient condition for invertibility.  
%
Since $\tr(\bH^u) = R$, this restricts $R < N_0/2$.
%
A similar conclusion is drawn for \VT~regression. 
%
\begin{remark} 
A benefit of PCR, in contrast to OLS, is that the nonsingularity conditions required for the jackknife and HRK covariance estimators can be controlled by the number of chosen principal components $k$. 
\end{remark} 

% PROBLEM 
%\subsubsection{Which Confidence Interval is Right for my Data---\HZ~or \VT?}
\subsubsection{All Models are Wrong, but are Some More Useful?}  
\label{sec:problem} 
%
The \HZ~and \VT~confidence intervals presented in Section~\ref{sec:ci.1} are rigorous under their respective models. 
%
Both models, however, are simplifications of reality. 
%
%Nevertheless, it is natural to ask if 
This begs the question: ``is one model more useful than the other?''
%
Towards providing a response, we underscore that the purpose of a confidence interval is to quantify uncertainties in the postulated model. 
%
While some assumptions require oracle information for verification, others can be checked from observed data. 
%
In our context, the data-friendly conditions correspond to Assumptions~\ref{assump:hz} and \ref{assump:vt} (i) and (iv.b). 
%

With this in mind, we inspect the confidence intervals. 
% 
Notably, each interval only depends on its particular in-sample error. 
%
The \HZ~error, $\bH^u_\perp \by_T$, quantifies the uncertainty in the \HZ~outcome model in Assumption~\ref{assump:hz} (i). 
%
Critically, \HZ~intervals overlook the \VT~error, $\bH^v_\perp \by_N$. 
%
While the \VT~error quantifies the uncertainty in the \VT~outcome model in Assumption~\ref{assump:vt} (i), it also checks Assumption~\ref{assump:hz} (iv.b). 
%
Hence, the \VT~error informs on the soundness of the \HZ~model, yet is completely neglected by the \HZ~intervals.  
%
The same arguments apply to \VT~intervals. 
%
Looking back, we have already seen these concerns play out in Figure~\ref{fig:teaser_inf}. 
%
It is clear from the \VT~OLS intervals that the \VT~model can grossly misrepresent reality through its fixation on one source of randomness. 
%
The \HZ~model suffers in an identical manner by the same logic. 

Conceptually, this reinforces the growing intuition that both regressions rely on time series and cross-sectional patterns for valid inference. 
%
Computationally, this suggests that both intervals should incorporate \HZ~and \VT~errors. 
%
For these reasons, we do not advocate for either model and instead look to fill in the gaps within each. 
%
% motivates the upcoming discussion. 

% UNIFIED 
\subsection{Inference under a Mixed Generative Model} 
\label{sec:unified} 
%
Motivated by our newfound insights, we present a new regression model with corresponding confidence intervals that account for uncertainties across time and space.  

% assumptions 
\subsubsection{Generative Model} \label{sec:mixed_model} 
%
At a high level, our postulated model mixes aspects of the \HZ~and \VT~models. 
%
To address the concerns laid out in Section~\ref{sec:problem}, the mixed model accounts for randomness along both dimensions of the data. 
%
This comes at the price of placing additional constraints on the stochastic properties of the errors. 

%In particular, we account for randomness along both dimensions of the data but place additional constraints on the stochastic properties of the errors. 

%
\begin{assumption}[Mixed generative model] \label{assump:hz_vt} 
%
Conditional on $\bY_0$, 
%
\begin{itemize} 
	\item[(i)] there exists $(\balpha^*, \bbeta^*)$ such that 
	\begin{enumerate}
		\item[(a)] $Y_{iT} = \sum_{t \le T_0} \alpha^*_t Y_{it} + \varepsilon_{iT}$ for $i \le N_0$
		\item[(b)] $Y_{Nt} = \sum_{i \le N_0} \beta^*_i Y_{it} + \varepsilon_{Nt}$ for $t \le T_0$ 
		\item[(c)] $Y_{NT} = \sum_{t \le T_0} \sum_{i \le N_0} \alpha^*_t \beta^*_i Y_{it} + \varepsilon_{NT}$.  
	\end{enumerate} 
	
%	(a) $\by_T = \bY_0 \balpha^* + \bvarepsilon_T$, (b) $\by_N = \bY'_0 \bbeta^* + \bvarepsilon_N$, and (c) $\Ex[Y_{NT}(0) | \bY_0] = \langle \bbeta^*, \bY_0 \balpha^* \rangle$. 
	
	\item[(ii)] $\varepsilon_{iT}$ and $\varepsilon_{Nt}$ are mean zero for $i \le N$ and $t \le T$.
	%{\em Strict exogeneity:} (a) $\Ex[\bvarepsilon_T | \bY_0] = \bzero$ and (b) $\Ex[\bvarepsilon_N | \bY_0] = \bzero$. 
	
	\item[(iii)] $\varepsilon_{iT}$ and $\varepsilon_{Nt}$ are independent over $i \le N$ and $t \le T$.
\end{itemize}
\end{assumption} 

% outcome model 
\smallskip 
\noindent 
{\bf (i) Outcome model.} 
%
%Roughly speaking, the mixed model makes weaker outcome modeling assumptions than the \HZ~and \VT~models.
%
Assumption~\ref{assump:hz_vt} (i.a) and (i.b) correspond to Assumptions~\ref{assump:hz} and \ref{assump:vt} (i), respectively. 
%
This explicitly models time series and cross-sectional patterns as two distinct sources of randomness. 
%
From the \HZ~perspective, Assumption~\ref{assump:hz_vt} (i.b) replaces Assumption~\ref{assump:hz} (iv), which removes cross-sectional uncertainties. 
%
Therefore, the statistical uncertainty of $\hY_{NT}(0)$ is governed by not only the construction of the regression model $\bhalpha$ from the control units' outcomes $(\by_T, \bY_0)$, but also the $\ell_2$-similarity between the treated units' lagged outcomes $\by_N$ with that of the control units $\bY_0$---these correspond to the in- and out-of-sample uncertainties, respectively. 
%
Analogous statements carry over to the \VT~perspective. 

Assumption~\ref{assump:hz_vt} (i.a) and (i.b) also justify Assumption~\ref{assump:hz_vt} (i.c). 
%
To see this, consider the \HZ~model with Assumption~\ref{assump:hz_vt} (i.b) in place of Assumption~\ref{assump:hz} (iv). 
%
Then, 
%
\begin{align}
	\Ex[Y_{NT}(0) | \bY_0] 
	&= \Ex\left[ \Ex[Y_{NT}(0) | \by_N, \bY_0] | \bY_0 \right]
	%= \Ex\left[ \Ex[Y_{NT}(0) | \by_N ] | \bY_0 \right] 
	= \Ex[ \langle \by_N, \balpha^* \rangle | \bY_0] 
	= \langle \bbeta^*, \bY_0 \balpha^* \rangle.
\end{align} 
%
Consider the \VT~DGP with Assumption~\ref{assump:hz_vt} (i.a) in place of Assumption~\ref{assump:vt} (iv). 
% 
Then, 
%
\begin{align} 
	\Ex[Y_{NT}(0) | \bY_0] 
	&= \Ex\left[ \Ex[Y_{NT}(0) | \by_T, \bY_0] | \bY_0 \right] 
	%= \Ex\left[ \Ex[Y_{NT}(0) | \by_T ] | \bY_0 \right] 
	= \Ex[ \langle \by_T, \bbeta^* \rangle | \bY_0] 
	= \langle \bbeta^*, \bY_0 \balpha^* \rangle. 
\end{align} 
%
The same conclusion is drawn from both perspectives. 

% strict exogeneity 
\smallskip 
\noindent 
{\bf (ii) Strict exogeneity.} 
%
Assumption~\ref{assump:hz_vt} (ii) combines Assumptions~\ref{assump:hz} and \ref{assump:vt} (ii). 
%
In words, it states that $\bY_0$ contains all measured confounders. 
%
In some sense, the \HZ~model already implies Assumption~\ref{assump:hz_vt} (ii.b) since $\by_N$ is treated deterministically; a similar logic applies to Assumption~\ref{assump:hz_vt} (ii.a) and the \VT~model. 

% independence 
\smallskip 
\noindent 
{\bf (iii) Independence.} 
%
Assumption~\ref{assump:hz_vt} (iii) combines Assumptions~\ref{assump:hz} and \ref{assump:vt} (iii). 
%
In words, it states that the errors are independent across time and space, which is more restrictive than Assumptions~\ref{assump:hz} and \ref{assump:vt} (iii) in isolation. 
%
We leave a proper analysis under dependent errors as future work, possibly by leveraging \cite{li2020}. 

% summary  
\smallskip 
\noindent 
{\bf Summary.} 
%
Assumption~\ref{assump:hz_vt} suggests the following DGP:
%
(i) sample $\bY_0$; 
(ii) sample $(\bvarepsilon_T, \bvarepsilon_N)$ independent of all other variables with $\Ex[\bvarepsilon_T | \bY_0] = \bzero$ and $\Ex[\bvarepsilon_N | \bY_0] = \bzero$;  
(iii) define $\by_T = \bY_0 \balpha^* + \bvarepsilon_T$, $\by_N = \bY'_0 \bbeta^* + \bvarepsilon_N$, and $Y_{NT}(0) = \langle \bbeta^*, \bY_0 \balpha^* \rangle + \varepsilon_{NT}$. 
%$\Ex[Y_{NT}(0) | \bY_0] = \langle \bbeta^*, \bY_0 \balpha^* \rangle$. 

% formal results 
\subsubsection{Asymptotic Properties} 
%
We study properties of $\hY_{NT}(0)$ under the mixed model. 
%We establish the \HZ~and \VT~asymptotic properties under the mixed DGP. 
%
%To this end, 
Let $\mu_0 = \Ex[Y_{NT}(0) | \bY_0]$. 
%
\begin{theorem} \label{thm:inference.hz_vt} 
%
Let Assumption~\ref{assump:hz_vt} hold.
%
%Conditioned on $\bY_0$ and 
Under suitable moment conditions,  
%
\begin{align}
	\frac{ \hY_{NT}(0) - \mu_0}{\sqrt{v_0}} \xrightarrow{d} \mathcal{N}(0,1),
\end{align}
%
where $v_0 = 
	 (\bH^u \bbeta^*)' \bSigma_T (\bH^u \bbeta^*)
	+ (\bH^v \balpha^*)' \bSigma_N (\bH^v \balpha^*)  
	+ \tr( \bY^\dagger_0 \bSigma_T (\bY'_0)^\dagger \bSigma_N)$. 
%
\end{theorem} 
%
Theorem~\ref{thm:inference.hz_vt} establishes that under the mixed model, the asymptotic variance of $\hY_{NT}(0)$ is controlled by time series patterns, cross-sectional patterns, and their interaction as quantified by the first three terms of $v_0$, respectively. 
%
The third term arises from the quadratic form of $\hY_{NT}(0)$ involving $(\by_N, \by_T)$, which are jointly random. 

%% core intuition 
%\smallskip 
%\noindent 
%{\bf Core intuition.} 
%%
%We discuss the intuition behind Theorem~\ref{thm:inference.hz_vt}. 
%%
%Consider the \HZ~perspective, which exploits time series patterns. 
%%
%If the treated unit is starkly different from the control units, e.g., $\by_N \notin \text{rowspan}(\bY'_0)$, then the regression model $\bhalpha$ learned on the control units $(\by_T, \bY_0)$ should not extrapolate to the treated unit $\by_N$ even if the treated period is similar to the pretreatment periods, e.g., $\by_T \in \text{rowspan}(\bY_0)$. 
%%
%This argument can be made precise through \eqref{eq:intuition}, and applies analogously for the \VT~perspective.
%%
%%Now, consider the \VT~perspective, which exploits cross-sectional correlations. 
%%%
%%If the treated period is starkly different from the pretreatment periods, e.g., $\by_T \notin \text{rowspan}(\bY_0)$, then the regression model $\bhbeta$ learned during the pretreatment periods $(\by_N, \bY_0)$ should not extrapolate to the treated period $\by_T$, even if the treated unit is similar to the control units, e.g., $\by_N \in \text{rowspan}(\bY'_0)$. 
%%
%%These arguments can be made precise through \eqref{eq:intuition}. 
%%
%Therefore, the \HZ~approach inevitably relies on cross-sectional patterns and the \VT~approach inevitably relies on time series patterns. 
%%---neither pattern is individually sufficient for inference. 
%%
%Accordingly, the prediction uncertainty should account for both sources of randomness. 
%%
%\begin{remark} 
%This intuition serves as the bedrock of this article and guides the upcoming discussions. 
%%
%Crucially, it is built upon the methodological framework of \HZ~and \VT~regressions, not our specific modeling assumptions. 
%%
%Therefore, our primary takeaways to follow should carry over to other inferential settings as well. 
%%
%\end{remark} 

% confidence interval  
\subsubsection{Confidence Interval} \label{sec:ci.2} 
%
We construct the mixed confidence interval as follows: for $\theta \in (0,1)$, 
%
\begin{align} \label{eq:ci.final}
	\text{(mixed confidence interval)} \quad 	
	\mu_0 &\in \left[ \hY_{NT}(0) ~\pm~ z_{\frac \theta 2} \sqrt{\hv_0} \right], 
\end{align}
%
where $\hv_0$ is the estimator of $v_0$.
%
%The \HZ~and \VT~regressions now share the same point prediction and confidence interval, as reflective of Theorem~\ref{thm:inference.hz_vt}.  
%
Motivated by Lemmas~\ref{lemma:inference.1}--\ref{lemma:inference.3}, we design
%
\begin{align}
	\hv_0  
	&= \hv_0^\hz 
	+ \hv_0^\vt
	-  \tr(\bY_0^\dagger \bhSigma_T (\bY'_0)^\dagger \bhSigma_N),  \label{eq:final_var_est} 
\end{align} 
%
where $(\hv_0^\hz, \hv_0^\vt)$ are given by \eqref{eq:hz_vt_specific_estimators}. 
%
We define $(\bhSigma_T, \bhSigma_N)$ using the estimators in Section~\ref{sec:ci.1}. 
%
We index $\hv_0$ by said estimators, e.g., $\hv^\jack_0$ uses $(\bhSigma^\jack_T, \bhSigma^\jack_N)$. 
%
In all cases, $\hv_0$ depends on both \HZ~and \VT~in-sample errors. 
%

We consider $\hv_0$ with respect to $v_0$. %\eqref{eq:final_var}. 
%
By construction, $\bhalpha = \bH^v \bhalpha$ and $\bhbeta = \bH^u \bhbeta$. 
%
To justify the negative trace in $\hv_0$, recall $\hv_0^\hz$ is a quadratic involving $(\by_N, \by_T)$. 
% 
Since both quantities are random, the expectation of $\hv_0^\hz$ induces an additional term that precisely corresponds to the interactive trace in $v_0$. %\eqref{eq:final_var}. 
%
The same property holds for $\hv_0^\vt$. 
%
Thus, $\hv_0$ corrects for this bias via the negative trace. 
%
We formalize this notion below. 
%
\begin{cor} \label{cor:var} 
%
Let Assumption~\ref{assump:hz_vt} hold. 
%
(i) Consider homoskedastic errors. 
%
Then, 
%(i) Under homoskedastic errors,   
$\Ex[\hv^\ehomo_0 | \bY_0] = v_0$. 
%
(ii) Consider heteroskedastic errors. 
%
(a) If $(\bH^u_\perp \circ  \bH^u_\perp \circ \bI)$ and $(\bH^v_\perp \circ  \bH^v_\perp \circ \bI)$ are nonsingular, then 
$
\Ex[\hv^\ejack_0 | \bY_0] \ge v_0. 
$
%
(b) If $(\bH^u_\perp \circ  \bH^u_\perp)$ and $(\bH^v_\perp \circ  \bH^v_\perp)$ are nonsingular,
then 
$\Ex[ \hv^\ehrk_0 | \bY_0] = v_0$. 
%
\end{cor} 
%
Corollary~\ref{cor:var} states that the homoskedastic and HRK estimators are unbiased while the jackknife estimator is conservative. 
%
Though these results hold in finite samples, they also only hold in expectation. 
%
For any particular realization, $\hv_0$ may exhibit undesirable characteristics. 
%
For instance, if  
$\tr(\bY_0^\dagger \bhSigma_T (\bY'_0)^\dagger \bhSigma_N) > \max\{\hv_0^\hz, \hv_0^\vt \}$, 
then $\hv_0 < \min\{\hv_0^\hz, \hv_0^\vt \}$, i.e., the mixed coverage will be smaller than both coverages. 
%
In fact, $\hv_0$ can even be negative if $\tr(\bY_0^\dagger \bhSigma_T (\bY'_0)^\dagger \bhSigma_N) > \hv_0^\hz + \hv_0^\vt$, which may occur if both \HZ~and \VT~in-sample errors are ``too large''. 
%
For these scenarios, one na\"ive solution is to modify $\hv_0$ as   
%
$\hv_0^{\text{mod}} = \hv_0^\hz + \hv_0^\vt$, which is conservative by Corollary~\ref{cor:var}. 
%
However, the latter case is arguably better resolved with a different estimator altogether. 

% IMPLICATION
\subsection{The Advantage of a Mixed Confidence Interval}  \label{sec:joint_advantage} 
%
Armed with our mixed interval, we explore its performance relative to \HZ~and \VT~intervals. 
%
Our investigation is based on three canonical case studies from the synthetic controls literature: (i) terrorism in Basque Country, (ii) California's Proposition 99 \citep{abadie2}, and (iii) the reunification of West Germany \citep{abadie4}. 
% 
We provide an overview of the results and primary messages in this section, and relegate details (e.g., implementation) to Appendix~\ref{sec:sim_emp}. 

\subsubsection{Background on Case Studies} 
%
\noindent 
{\bf California Proposition 99.} 
This study examines the effect of California's Proposition 99, an anti-tobacco legislation, on its tobacco consumption. 
%
The panel data contains per capita cigarette sales of $N = 39$ U.S. states across $T=31$ years. 
%
There are $T_0=18$ pretreatment observations and $N_0 = 38$ control units. 
%
Our interest is to estimate California's cigarette sales in the absence of Proposition 99. 
%

\smallskip
\noindent
{\bf Reunification in West Germany.}
%
This study examines the economic impact of the 1990 reunification in West Germany.   
%
Our panel data contains per capita GDP of $N=17$ countries across $T=44$ years. 
%
There are $T_0 = 30$ pretreatment observations and $N_0=16$ control units. 
%
Similar to the Basque study, our interest here is to estimate West Germany's GDP in the absence of reunification. 
%

% SIMULATIONS
\subsubsection{Data-Inspired Simulation Studies} \label{sec:simulations.1} 
%
To assess the relative performances in a realistic environment, we calibrate our simulations to the two case studies. 
%
%For a proper analysis, 
We perform model checks for Assumption~\ref{assump:hz_vt}, which indirectly checks Assumptions \ref{assump:hz}--\ref{assump:vt} as discussed in Section~\ref{sec:mixed_model}.

% DGP 
\smallskip 
\noindent 
{\bf Data generating process.} 
%
In each study, we hold out a portion of the observed control data as a ``test'' set. 
%
Thus, we only consider the pretreatment outcomes, e.g., the GDP of all Spanish regions prior to the outset of terrorism. % in Basque Country. 
%
These observations constitute our ground truth of {\em expected} potential outcomes. 
%
In congruence with the article, we focus on the single treated unit and time period setting. 
%
We retain the actual treated unit, e.g., Basque Country, but artificially designate the final pretreatment period, e.g., one year prior to the outset of terrorism, as the pseudo treated period. 
%

We set our causal estimand as $\mu_0 = Y_{NT_0}$, e.g., Basque Country's GDP one year prior to the outset of terrorism. 
%
We fix $\mu_0$ and $\bY_0$, which we temporarily redefine as $\bY_0 = [Y_{it}: i \le N_0, t < T_0]$; note that $\bY_0$ excludes outcomes in the actual final pretreatment period. 
%
For stability analysis, we randomly perturb the treated unit's pretreatment outcomes and the control units' pseudo treated period outcomes.   
%
In each simulation repeat, we sample $\by_N$ from a multivariate Gaussian distribution with mean $[Y_{Nt}: t < T_0]$ and variance $\bSigma_N = \sigma^2_N \bI$, where $\sigma^2_N$ is the observed standard error of $[Y_{Nt}: t < T_0]$. 
%
We sample $\by_{T_0}$ analogously with respect to $[Y_{iT_0}: i \le N_0]$. 
%
%$(\by_N, \by_{T_0})$ from their respective Gaussian distributions whose means are given by $[Y_{Nt}: t < T_0]$ and $[Y_{iT_0}: i \le N_0]$, respectively, and . 
%
Note that this design choice respects Assumption~\ref{assump:hz_vt} (ii)--(iii). 
%
By construction, our simulated DGPs are calibrated to the underlying DGPs of the case studies since (i) $(\mu_0, \bY_0)$ and (ii) the expected values of $(\by_N, \by_{T_0})$ are all observed quantities. 
%
%Therefore, our conclusions to follow may be transferrable to other practical settings. 

% RESULTS
\smallskip 
\noindent 
{\bf Simulation results.} 
%
We conduct 500 replications of the above DGP for each study. 
% 

% PREDICTION ERRORS
\smallskip 
\noindent 
{\em I: Prediction errors.} 
%
%We first check the quality of the linear outcome model of Assumption~\ref{assump:hz_vt} (i). 
%
Table~\ref{table:bias_rmse} summarizes the OLS and PCR prediction errors across four metrics: 
(i-ii) \HZ~and \VT~in-sample errors,  
(iii-iv) out-of-sample bias and root-mean-squared-error (RMSE). 
%
For ease of comparison, we normalize all four metrics by the $\ell_2$-norm of the true outcomes. 
%
With the exception of the Basque study, our findings suggest that linear predictors adequately fit the underlying outcomes, i.e., Assumption~\ref{assump:hz_vt} (i) is reasonable. 
%
We probe the Basque study in the following evaluation. 

%With the exception of the high out-of-sample bias and RMSE for OLS in the Basque study, 
%With the exception of the Basque study, our findings suggest that linear predictors adequately fit the underlying outcomes, i.e., Assumption~\ref{assump:hz_vt} (i) is reasonable. 
%Our findings suggest that linear predictors adequately fit the underlying outcomes, 
%%The low errors suggest that the true outcome model is approximately linear, 
%i.e., Assumption~\ref{assump:hz_vt} (i) is reasonable. 
%
%The notable exceptions are the high bias and RMSE for OLS in the Basque study, which is unsurprising given Figure~\ref{fig:teaser_est}. 

% OLS BIAS + RMSE 
\begin{table} [!t]
\centering 
%%\smaller 
\caption{Average prediction errors for OLS and PCR across 500 simulation replications.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study} 
& \multicolumn{4}{c}{OLS} 
& \multicolumn{4}{c}{PCR}  
\\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \HZ~error   & \VT~error	& Bias   & RMSE  
& \HZ~error   & \VT~error	& Bias   & RMSE 
\\
\cmidrule(){1-9} 
Basque
& $0.08$    & $0.00$		& $-3.30$    & $261$    
& $0.22$    & $0.16$ 	& $0.01$    & $0.15$      
\\
California
& $0.04$    & $0.00$ 	& $0.00$    & $0.01$    
& $0.05$    & $0.03$ 	& $0.01$    & $0.03$   
\\ 
W. Germany
& $0.00$    & $0.01$ 	& $-0.01$    & $0.01$    
& $0.01$    & $0.01$ 	& $-0.01$    & $0.01$     
\\
\bottomrule
\end{tabular}
\label{table:bias_rmse}
\end{table} 

% coverage rates 
\smallskip 
\noindent 
{\em II: Coverage.} 
%
After checking our modeling assumptions, we are ready to compare the performances of the \HZ, \VT, mixed, and modified mixed intervals. 
%
Tables~\ref{table:ols_coverage} and \ref{table:pcr_coverage} display the coverage probabilities (CP) and average lengths (AL) for nominal 95\% confidence intervals of OLS and PCR, respectively, in regards to $\mu_0$. 
%
We normalize the coverage length by the magnitude of the corresponding prediction value. 

For each OLS study, either the \HZ~or \VT~interval is degenerate.
% 
Subsequently, the mixed interval achieves the same coverage as the non-degenerate interval.  
%
This phenomena is highlighted by the Basque study. 
%
Despite alarmingly high prediction errors, the \VT~intervals fail to capture the erroneous behavior of the OLS predictions. 
%
By comparison, the large ALs of the \HZ~and mixed intervals vehemently put into question the credibility of the OLS prediction. 
%
Although any sensible researcher would discard these OLS estimates even without aid from a confidence interval, this example showcases that the mixed interval safeguards the researcher from non-degeneracy, provided at least one of the two independent intervals is non-degenerate. 

Moving to PCR, we observe that while both \HZ~and \VT~intervals are non-degenerate, 
the mixed interval coverage is generally closer to the nominal coverage. 
%
The exception to this trend is the Basque study, which presents another useful lesson. 
%
Here, the CPs of the \HZ~and \VT~jackknife intervals are larger than that of the mixed jackknife interval. 
%
This illustrates the fragility of the mixed interval when both the \HZ~and \VT~in-sample errors are large, as noted in Section~\ref{sec:ci.2}. 
%
The modified mixed interval circumvents this concern but is still far from optimal. 

%However, their CPs can be relatively low compared to that of the mixed intervals. 
%With all things considered, our simulations provide evidence that the mixed interval coverage is generally closer to the nominal coverage compared to \HZ~and \VT~intervals, which often undercover. 

%  OLS COVERAGE
\begin{table} [!t]
\centering 
\caption{OLS coverage for nominal 95\% confidence intervals across 500 replications.}
\begin{tabular}{@{}ccccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study}
& \multicolumn{3}{c}{OLS Homoskedastic} 
& \multicolumn{3}{c}{OLS Jackknife}   
\\ 
\cmidrule(l){2-4} 
\cmidrule(l){5-7}
& \HZ   & \VT   & Mixed 
& \HZ   & \VT   & Mixed  	
\\
\cmidrule(){1-7} 
Basque (CP)
% ols
& $0.81$    & $0.00$    & $0.81$ 
& $0.99$    & $0.00$    & $0.99$ 
\\ 
Basque (AL)
% ols
& $14.2$    & $0.00$    & $14.2$ 
& $211$     & $0.00$    & $211$ 
\\
\cmidrule(){1-7} 
California (CP) 
% ols
& $0.90$    & $0.00$    & $0.90$ 
& $0.99$    & $0.00$    & $0.99$ 
\\ 
California (AL)
% ols
& $0.28$    & $0.00$    & $0.28$ 
& $0.54$    & $0.00$    & $0.54$ 
\\
\cmidrule(){1-7} 
W. Germany (CP)
% ols
& $0.00$    & $0.90$    & $0.90$ 
& $0.00$    & $0.98$    & $0.98$ 
\\ 
W. Germany (AL)
% ols
& $0.00$    & $0.04$    & $0.04$ 
& $0.00$    & $0.08$    & $0.08$ 
\\
\bottomrule
\end{tabular}
\label{table:ols_coverage}
\end{table}

% PCR COVERAGE
\begin{table} [!t]
\centering 
\caption{PCR coverage for nominal 95\% confidence intervals across 500 replications.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study}   
& \multicolumn{4}{c}{PCR Homoskedastic} 
& \multicolumn{4}{c}{PCR Jackknife}  
\\ 
\cmidrule(l){2-5} 
\cmidrule(l){6-9}
& \HZ   & \VT   & Mixed     & Mod. 
& \HZ   & \VT   & Mixed  	& Mod. 
\\
\cmidrule(){1-9} 
Basque (CP)
% pcr
& $0.80$    & $0.84$    & $0.92$    & $0.95$ 
& $0.82$    & $0.85$    & $0.80$    & $0.97$
\\ 
Basque (AL)
% pcr
& $0.39$    & $0.45$    & $0.54$    & $0.56$ 
& $0.57$    & $0.54$    & $0.62$    & $0.75$
\\
\cmidrule(){1-9}
California (CP) 
% pcr
& $0.70$    & $0.94$    & $0.96$    & $0.96$ 
& $0.76$    & $0.90$    & $0.96$    & $0.96$
\\ 
California (AL)
% pcr
& $0.06$    & $0.12$    & $0.13$    & $0.13$ 
& $0.07$    & $0.12$    & $0.14$    & $0.14$
\\
\cmidrule(){1-9} 
W. Germany (CP)
% pcr
& $0.65$    & $0.94$    & $0.97$    & $0.97$ 
& $0.74$    & $0.86$    & $0.96$    & $0.96$
\\ 
W. Germany (AL)
% pcr
& $0.02$    & $0.03$    & $0.03$    & $0.03$ 
& $0.02$    & $0.03$    & $0.04$    & $0.04$
\\
\bottomrule
\end{tabular}
\label{table:pcr_coverage}
\end{table}


% EMPIRICAL ILLUSTRATIONS
\subsubsection{Empirical Illustrations} 
%
Next, we apply our uncertainty estimators to analyze the three case studies.  
%
We construct an illustrative narrative around Figures~\ref{fig:ols_homo}--\ref{fig:pcr_jack} with the help of three researchers: one \HZ, one \VT, and one ``agnostic''. 
%
We note that the following discussion only concerns the mixed interval $\hv_0$ as defined in \eqref{eq:final_var_est}.

%
Our three researchers begin with the Basque study and use OLS. 
%
Despite their different beliefs of the underlying DGP,
they independently arrive at the same counterfactual trajectory that suggests terrorism is net positive for the Basque economy. 
%
Although the OLS predictions are clearly implausible, the \VT~intervals shown in Figures~\ref{fig:basque_vt_homo} and \ref{fig:basque_vt_jack} reveal zero uncertainty. 
%
In contrast, the \HZ~intervals shown in Figures~\ref{fig:basque_hz_homo} and \ref{fig:basque_hz_jack} reflect massive levels of uncertainty, which resonates with intuition. 
%
Finally, the agnostic researcher who values both of their colleagues' perspectives, employs the mixed confidence intervals shown in Figures~\ref{fig:basque_mixed_homo} and \ref{fig:basque_mixed_jack}. 
%
Like the \HZ~intervals, the mixed intervals cast doubt on the OLS estimates. 
%
The researchers observe similar but less pronounced findings in the California study.  

%The three researchers then transition to the California study. 
%%
%Like the Basque study, the \HZ~intervals shown in Figures~\ref{fig:prop99_hz_homo} and \ref{fig:prop99_hz_jack} increase over time while the \VT~intervals shown in Figures~\ref{fig:prop99_vt_homo} and \ref{fig:prop99_vt_jack} are degenerate. 
%%
%As such, the mixed intervals shown in Figures~\ref{fig:prop99_mixed_homo} and \ref{fig:prop99_mixed_jack} match the \HZ~intervals. 

In the West Germany study, however, the \HZ~intervals shown in Figures~\ref{fig:germany_hz_homo} and \ref{fig:germany_hz_jack} are now the degenerate cases. 
%
The \VT~intervals shown in Figures~\ref{fig:germany_vt_homo} and \ref{fig:germany_vt_jack}, on the other hand, expand over time. 
%
Consequently, the mixed intervals in Figures~\ref{fig:germany_mixed_homo} and \ref{fig:germany_mixed_jack} match the \VT~intervals. 
%
Our researchers observe a similar storyline when they apply PCR to the three studies, as visualized in Figures~\ref{fig:pcr_homo} and \ref{fig:pcr_jack}. 

Through our researchers' experiences, we observe that the mixed intervals exhibit desirable robustness properties relative to \HZ~and \VT~intervals. 
%
Combined with our simulation studies and discussion in Section~\ref{sec:problem}, we conclude that the mixed interval is generally advantageous over \HZ~and \VT~intervals in this respect. 
%the mixed interval can relieve the burden on the researcher of deliberating between which interval---the \HZ~or the \VT---to trust. 
%
%Put differently, 
%the mixed interval can safeguard a researcher from drawing causal conclusions from the ``less informative'' interval.
%%
%The robustness feature of the mixed interval is a direct consequence of accounting for both sources of uncertainty in the underlying DGP. 

% OLS HOMOSKEDASTIC
\begin{figure} [H]
	\centering 
	% *** BASQUE ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:basque_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:basque_vt_homo} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:basque_mixed_homo}
	\end{subfigure} 	
	\\
	% *** CALIFORNIA ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:prop99_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:prop99_vt_homo}
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:prop99_mixed_homo}
	\end{subfigure} 	
	\\
	% *** GERMANY *** 
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:germany_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:germany_vt_homo} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:germany_mixed_homo}
	\end{subfigure} 	
	\caption{
	%
	OLS estimates with homoskedastic confidence intervals. 
	Columns are indexed by the type of confidence interval, e.g., \HZ. 
	(Top) Basque Country study. 
	(Middle) California study. 
	(Bottom) West Germany study.  
	}
	\label{fig:ols_homo} 
\end{figure}   

% OLS JACKKNIFE
\begin{figure} [H]
	\centering 
	% *** BASQUE ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:basque_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:basque_vt_jack} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/ols_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:basque_mixed_jack}
	\end{subfigure} 	
	\\
	% *** CALIFORNIA ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:prop99_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:prop99_vt_jack}
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/ols_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:prop99_mixed_jack}
	\end{subfigure} 	
	\\
	% *** GERMANY *** 
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:germany_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:germany_vt_jack} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/ols_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:germany_mixed_jack}
	\end{subfigure} 	
	\caption{
	%
	OLS estimates with jackknife confidence intervals. 
	Columns are indexed by the type of confidence interval, e.g., \HZ. 
	(Top) Basque Country study. 
	(Middle) California study. 
	(Bottom) West Germany study.  
	}
	\label{fig:ols_jack} 
\end{figure} 

% PCR HOMOSKEDASTIC
\begin{figure} [H]
	\centering 
	% *** BASQUE ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:pcr_basque_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:pcr_basque_vt_homo} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:pcr_basque_mixed_homo}
	\end{subfigure} 	
	\\
	% *** CALIFORNIA ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:pcr_prop99_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:pcr_prop99_vt_homo}
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:pcr_prop99_mixed_homo}
	\end{subfigure} 	
	\\
	% *** GERMANY *** 
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_hz_homoskedastic.png}
		\caption{\HZ.} 
		\label{fig:pcr_germany_hz_homo}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_vt_homoskedastic.png}
		\caption{\VT.} 
		\label{fig:pcr_germany_vt_homo} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_mixed_homoskedastic.png}
		\caption{Mixed.} 
		\label{fig:pcr_germany_mixed_homo}
	\end{subfigure} 	
	\caption{
	%
	PCR estimates with homoskedastic confidence intervals. 
	Columns are indexed by the type of confidence interval, e.g., \HZ. 
	(Top) Basque Country study. 
	(Middle) California study. 
	(Bottom) West Germany study.  
	}
	\label{fig:pcr_homo} 
\end{figure}   

% PCR JACKKNIFE
\begin{figure} [H]
	\centering 
	% *** BASQUE ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:pcr_basque_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:pcr_basque_vt_jack} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/basque/pcr_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:pcr_basque_mixed_jack}
	\end{subfigure} 	
	\\
	% *** CALIFORNIA ***
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:pcr_prop99_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:pcr_prop99_vt_jack}
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99/pcr_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:pcr_prop99_mixed_jack}
	\end{subfigure} 	
	\\
	% *** GERMANY *** 
	% HZ-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_hz_jackknife.png}
		\caption{\HZ.} 
		\label{fig:pcr_germany_hz_jack}
	\end{subfigure} 
	% VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_vt_jackknife.png}
		\caption{\VT.} 
		\label{fig:pcr_germany_vt_jack} 
	\end{subfigure} 
	% HZ-VT-homo
	\begin{subfigure}[b]{0.32\textwidth}
		\includegraphics[width=\linewidth]
		{images/germany/pcr_mixed_jackknife.png}
		\caption{Mixed.} 
		\label{fig:pcr_germany_mixed_jack}
	\end{subfigure} 	
	\caption{
	%
	PCR estimates with jackknife confidence intervals. 
	Columns are indexed by the type of confidence interval, e.g., \HZ. 
	(Top) Basque Country study. 
	(Middle) California study. 
	(Bottom) West Germany study.  
	}
	\label{fig:pcr_jack} 
\end{figure} 

\newpage 
% DESIGN BASED
\subsection{Design-Based Inference} 
%
We transfer our insights extracted from the model-based perspective to the design-based framework. 
%
To this end, we consider the related work of \cite{guido_inf}, which studies synthetic controls methods under design-based assumptions. 
%
The paper focuses on the causal effect for a single treated unit and time period pair: 
%
\begin{align}
	\tau = \sum_{i \le N} \sum_{t \le T} U_i V_t \big(Y_{it}(1) - Y_{it}(0) \big),
\end{align} 
%
where $U_i \in \{0,1\}$ and $V_t \in \{0,1\}$ indicate the treated unit and time period, respectively,
e.g., $U_N = 1$ and $V_T = 1$ if unit $N$ is treated at time $T$.  
%
There are three assignment mechanisms: 
(i) random assignment of the treated period, $\Pb(V_t = 1) = 1/T$;
(ii) random assignment of the treated unit, $\Pb(U_i = 1) = 1/N$;   
and (iii) random assignment of both. 
%
The potential outcomes are fixed throughout. 
%
Notably, (i) and (ii) are related to the ``in-time'' and ``in-space'' placebo tests proposed in \cite{abadie2, abadie4}. 
%

Mechanisms (i)--(iii) map to Assumptions~\ref{assump:hz}--\ref{assump:hz_vt} of this article. 
%
Accordingly, under (i), $\Ex[\tau] = (1/T) \sum_{i \le N} \sum_{t \le T} U_i (Y_{it}(1) - Y_{it}(0))$ is the average effect for the treated unit across all $T$ time periods, which the authors call the ``\HZ''~effect. 
%
Under (ii), $\Ex[\tau] = (1/N) \sum_{i \le N} \sum_{t \le T} V_t (Y_{it}(1) - Y_{it}(0))$ is the average effect across all $N$ units in the treated period, also called the ``\VT''~effect. 
%
Under (iii), $\Ex[\tau] = 1/(NT) \sum_{i \le N} \sum_{t \le T} (Y_{it}(1) - Y_{it}(0))$ is the average effect across all unit and time period pairs, which we coin the ``mixed'' effect. 
%
In view of Section~\ref{sec:joint_advantage}, mechanism (iii) has the advantage of offering two choices for conducting inference. 

% RIDGE 
\subsection{Extension to Other Estimators}
%
Any estimator, regardless of its placement in the symmetric or asymmetric class, can be studied from the mixed modeling perspective. 
%
In doing so, the variance of the corresponding counterfactual prediction can be derived to construct appropriate mixed confidence intervals. 
%
We leave a thorough analysis of other estimators as an interesting line of future inquiry. 

%Properties for ridge regression and the asymmetric estimators can be established under the mixed generative model or a variant thereof to derive corresponding mixed confidence intervals. 
%

%An important facet of (iii) is that it offers two choices for conducting inference. 

%

%%
%If the treated unit is randomly selected, i.e., $\Pb(U_i = 1) = 1/N$, then $\Ex[\tau] = (1/N) \sum_{i \le N} \sum_{t \le T} V_t (Y_{it}(1) - Y_{it}(0))$ is the average effect for all $N$ units in the treated period, which the authors coin the ``vertical'' effect. 
%%
%If the treated period is randomly selected, i.e., $\Pb(V_t = 1) = 1/T$, then $\Ex[\tau] = (1/T) \sum_{i \le N} \sum_{t \le T} U_i (Y_{it}(1) - Y_{it}(0))$ is the average effect for the treated unit over all $T$ periods, the ``horizontal'' effect. 
%%
%If both are randomly selected, then $\Ex[\tau] = 1/(NT) \sum_{i \le N} \sum_{t \le T} (Y_{it}(1) - Y_{it}(0))$ is the average effect across all unit and time period pairs. 
%
%Within this framework, our article advocates for the third treatment assignment mechanism as it offers two choices for conducting inference. 



%There are three assignment mechanisms of interest: 
%(i) random assignment of the treated unit, $\Pb(U_i = 1) = 1/N$;  
%(ii) random assignment of the treated period, $\Pb(V_t = 1) = 1/T$; 
%(iii) random assignment of both. 
%%
%Under (i), $\Ex[\tau] = (1/N) \sum_{i \le N} \sum_{t \le T} V_t (Y_{it}(1) - Y_{it}(0))$ measures the average effect for all $N$ units in the treated period, which the authors coin the ``vertical'' effect. 
%%
%Under (ii), $\Ex[\tau] = (1/T) \sum_{i \le N} \sum_{t \le T} U_i (Y_{it}(1) - Y_{it}(0))$ measures the average effect for the treated unit overall $T$ periods, the ``horizontal'' effect. 
%%
%Under (iii), $\Ex[\tau] = 1/(NT) \sum_{i \le N} \sum_{t \le T} (Y_{it}(1) - Y_{it}(0))$ measures the average effect across all unit and time period pairs. 

%% OLS JACKKNIFE
%\begin{figure} [!p]
%	\centering 
%	% OLS HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%		\label{fig:basque_hz_homo}
%	\end{subfigure} 
%	% OLS VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%		\label{fig:basque_vt_homo} 
%	\end{subfigure} 
%	% OLS HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%		\label{fig:basque_mixed_homo}
%	\end{subfigure} 	
%	% OLS HZ-jack
%	\\
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%		\label{fig:basque_hz_jack}
%	\end{subfigure} 
%	% OLS VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%		\label{fig:basque_vt_jack} 
%	\end{subfigure} 
%	% OLS HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/basque/ols_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%		\label{fig:basque_mixed_jack}
%	\end{subfigure} 
%	\\
%	% OLS HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%		\label{fig:germany_hz_homo}
%	\end{subfigure} 
%	% OLS VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%		\label{fig:germany_vt_homo} 
%	\end{subfigure} 
%	% OLS HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%		\label{fig:germany_mixed_homo}
%	\end{subfigure} 	
%	% OLS HZ-jack
%	\\
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%		\label{fig:germany_hz_jack}
%	\end{subfigure} 
%	% OLS VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%		\label{fig:germany_vt_jack} 
%	\end{subfigure} 
%	% OLS HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\includegraphics[width=\linewidth]
%		{images/germany/ols_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%		\label{fig:germany_mixed_jack}
%	\end{subfigure} 
%	\caption{
%	%
%	OLS estimates and confidence intervals. 
%	The top two rows correspond to the Basque study while the bottom two rows correspond to the West Germany study. 
%	We index rows by the covariance estimator, e.g., jackknife, and the columns by the type of confidence interval, e.g., \HZ.   
%	}
%	\label{fig:basque_ci} 
%\end{figure}   
%
%% PCR HOMOSKEDASTIC
%\begin{figure} [!p]
%	\centering 
%	% PCR HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%	\end{subfigure} 
%	% PCR VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%	\end{subfigure} 
%	% PCR HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%	\end{subfigure} 	
%	\\
%	% PCR HZ-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%	\end{subfigure} 
%	% PCR VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%	\end{subfigure} 
%	% PCR HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%	\end{subfigure} 	
%	\\ 
%	% PCR HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%		\label{fig:germany_hz_homo.pcr}
%	\end{subfigure} 
%	% PCR VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%	\end{subfigure} 
%	% PCR HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%	\end{subfigure} 	
%	\\
%	% PCR HZ-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%	\end{subfigure} 
%	% PCR VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%	\end{subfigure} 
%	% PCR HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%		\label{fig:germany_mixed_jack.pcr}
%	\end{subfigure} 	
%	\caption{
%	%
%	PCR estimates and confidence intervals. 
%	The top two rowscorrespond to the Basque study while the bottom two rows correspond to the West Germany study. 
%	We index rows by the covariance estimator, e.g., jackknife, and the columns by the type of confidence interval, e.g., \HZ.
%	}
%	\label{fig:basque_ci.pcr} 
%\end{figure} 
%
%% PCR JACKKNIFE
%\begin{figure} [!p]
%	\centering 
%	% PCR HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%	\end{subfigure} 
%	% PCR VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%	\end{subfigure} 
%	% PCR HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%	\end{subfigure} 	
%	\\
%	% PCR HZ-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%	\end{subfigure} 
%	% PCR VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%	\end{subfigure} 
%	% PCR HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/basque/pcr_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%	\end{subfigure} 	
%	\\ 
%	% PCR HZ-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_hz_homoskedastic.png}
%		\caption{\HZ~homoskedastic.} 
%		\label{fig:germany_hz_homo.pcr}
%	\end{subfigure} 
%	% PCR VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_vt_homoskedastic.png}
%		\caption{\VT~homoskedastic.} 
%	\end{subfigure} 
%	% PCR HZ-VT-homo
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_mixed_homoskedastic.png}
%		\caption{Mixed homoskedastic.} 
%	\end{subfigure} 	
%	\\
%	% PCR HZ-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_hz_jackknife.png}
%		\caption{\HZ~jackknife.} 
%	\end{subfigure} 
%	% PCR VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_vt_jackknife.png}
%		\caption{\VT~jackknife.} 
%	\end{subfigure} 
%	% PCR HZ-VT-jack
%	\begin{subfigure}[b]{0.32\textwidth}
%		\centering 
%		\includegraphics[width=\linewidth]
%		{images/germany/pcr_mixed_jackknife.png}
%		\caption{Mixed jackknife.} 
%		\label{fig:germany_mixed_jack.pcr}
%	\end{subfigure} 	
%	\caption{
%	%
%	PCR estimates and confidence intervals. 
%	The top two rowscorrespond to the Basque study while the bottom two rows correspond to the West Germany study. 
%	We index rows by the covariance estimator, e.g., jackknife, and the columns by the type of confidence interval, e.g., \HZ.
%	}
%	\label{fig:basque_ci.pcr} 
%\end{figure} 
%
%
%


==> content/proofs_doublerobust.tex <==
%\section{Proofs for Doubly Robust Estimators} 

%% SDID 
%\subsection{Proof of Theorem~\ref{thm:sdid}: Doubly robust estimators} 
%
%\begin{proof}
%% 
%We begin with the OLS setting. 
%%
%Recall that $\hY^\hz_{NT}(0)  = \langle \by_N, \bhalpha \rangle$ and $\hY^\vt_{NT}(0) = \langle \by_T, \bhbeta \rangle$. 
%%
%By Theorem~\ref{thm:equivalent},
%%
%\begin{align}
%	\hY^\hz_{NT}(0)  = \hY^\vt_{NT}(0) = \langle \by_N, \bY_0^\dagger \by_T \rangle,
%\end{align} 
%%
%thus $\bhalpha = \bY_0^\dagger \by_T$ and $\bhbeta = (\bY_0')^\dagger \by_N$. 
%%
%Returning to \eqref{eq:sdid}, we obtain
%%
%\begin{align}
%	\hY^\sdid_{NT}(0) &= \hY^\asc_{NT}(0) =  \langle \by_T, \bhbeta \rangle + \langle \by_N, \bhalpha \rangle - \langle \bhalpha, \bY_0' \bhbeta \rangle  
%	= 2 \hY^\hz_{NT}(0) - \langle  \bhalpha, \bY_0' \bhbeta \rangle. \label{eq:sdid.0} 
%\end{align} 
%%
%Recall $(\bY_0')^\dagger  = (\bY_0^\dagger)'$. 
%%
%Therefore,  
%%
%\begin{align}
% 	\langle  \bhalpha, \bY_0' \bhbeta \rangle &= \by'_T(\bY_0')^\dagger \bY_0' (\bY_0')^\dagger \by_N 
%%	\\ &= \by'_T(\bU \bS^{-1} \bV') \bV \bS \bU' (\bU \bS^{-1} \bV') \by_N 
%%	\\ &=  \by'_T(\bU \bS^{-1} \bV') \by_N 
%	= \by'_T(\bY_0')^\dagger \by_N 
%	= \by'_T \bhbeta. \label{eq:sdid.1} % = \hY^\hz_{NT}(0). 
%\end{align} 
%%
%Plugging \eqref{eq:sdid.1} into \eqref{eq:sdid.0}, we conclude 
%%
%\begin{align}
%	\hY^\sdid_{NT}(0) &= \hY^\asc_{NT}(0) = 2 \hY^\hz_{NT}(0) - \hY^\hz_{NT}(0)
%	= \hY^\hz_{NT}(0) = \hY^\vt_{NT}(0). 
%\end{align}  
%% 
%Now, observe that the same arguments above hold when $\bY_0^{(k)}$ takes the place of $\bY_0$ for any $k < R$. 
%%
%Therefore, the same reduction can be derived for PCR. 
%\end{proof} 



%% ERM 
%\subsection{Proof of Proposition~\ref{prop:erm}} 
%
%\begin{proof}
%
%\end{proof} 








==> content/proofs_doublyrobust.tex <==
% SDID 
\section{Proofs for The Researcher's Guide to Panel Data} 
%
\subsection{Proof of Corollary~\ref{cor:sdid}} %: Doubly Robust Estimators} 

\begin{proof}
% 
We begin with the OLS setting. 
%
Recall that $\hY^\hz_{NT}(0)  = \langle \by_N, \bhalpha \rangle$ and $\hY^\vt_{NT}(0) = \langle \by_T, \bhbeta \rangle$. 
%
By Theorem~\ref{thm:equivalent},
%
\begin{align}
	\hY^\hz_{NT}(0)  = \hY^\vt_{NT}(0) = \langle \by_N, \bY_0^\dagger \by_T \rangle,
\end{align} 
%
thus $\bhalpha = \bY_0^\dagger \by_T$ and $\bhbeta = (\bY_0')^\dagger \by_N$. 
%
Returning to \eqref{eq:sdid}, we obtain
%
\begin{align}
	\hY^\sdid_{NT}(0) &= \hY^\asc_{NT}(0) =  \langle \by_T, \bhbeta \rangle + \langle \by_N, \bhalpha \rangle - \langle \bhalpha, \bY_0' \bhbeta \rangle  
	= 2 \hY^\hz_{NT}(0) - \langle  \bhalpha, \bY_0' \bhbeta \rangle. \label{eq:sdid.0} 
\end{align} 
%
Recall $(\bY_0')^\dagger  = (\bY_0^\dagger)'$. 
%
Therefore,  
%
\begin{align}
 	\langle  \bhalpha, \bY_0' \bhbeta \rangle &= \by'_T(\bY_0')^\dagger \bY_0' (\bY_0')^\dagger \by_N 
%	\\ &= \by'_T(\bU \bS^{-1} \bV') \bV \bS \bU' (\bU \bS^{-1} \bV') \by_N 
%	\\ &=  \by'_T(\bU \bS^{-1} \bV') \by_N 
	= \by'_T(\bY_0')^\dagger \by_N 
	= \by'_T \bhbeta. \label{eq:sdid.1} % = \hY^\hz_{NT}(0). 
\end{align} 
%
Plugging \eqref{eq:sdid.1} into \eqref{eq:sdid.0}, we conclude 
%
\begin{align}
	\hY^\sdid_{NT}(0) &= \hY^\asc_{NT}(0) = 2 \hY^\hz_{NT}(0) - \hY^\hz_{NT}(0)
	= \hY^\hz_{NT}(0) = \hY^\vt_{NT}(0). 
\end{align}  
% 
Now, observe that the same arguments above hold when $\bY_0^{(k)}$ takes the place of $\bY_0$ for any $k < R$. 
%
Therefore, the same reduction can be derived for PCR. 
\end{proof} 

==> content/proofs_guide.tex <==
\section{Proofs for Diagnosing Counterfactual Models} 

\subsection{Proof of Proposition~\ref{prop:erm}} 
\begin{proof}
For any $\btx$, we have  
\begin{align} \label{eq:00} 
	\bhh(\btx) - \bbf^*(\btx) = ( \bhh(\btx) - \bh^*(\btx) ) + ( \bh^*(\btx) - \bbf^*(\btx) ). 
\end{align}
%
Observe that
%
\begin{align}
	\bhh(\btx) - \bh^*(\btx) &= \langle \bhh - \bh^*, \phi(\btx) \rangle
	\\ &= \langle \bP(\bhh - \bh^*) + \bP_\perp(\bhh - \bh^*), \phi(\btx) \rangle  
	\\ &= \langle \bP(\bhh - \bh^*), \phi(\btx) \rangle  + \langle \bP_\perp(\bhh - \bh^*), \phi(\btx) \rangle. 
\end{align}
% 
By \eqref{eq:representer} (Representer Theorem), $\bP \bhh = \bhh$ and $\bP_\perp \bhh = 0$. 
%
As a result,
%
\begin{align}
	\bhh(\btx) - \bh^*(\btx) &= \langle \bP(\bhh - \bh^*), \phi(\btx) \rangle  - \langle \bP_\perp \bh^*, \phi(\btx) \rangle
	\\ &= \langle \bhh - \bP \bh^*, \phi(\btx) \rangle - \langle \bh^*, \bP_\perp \phi(\btx) \rangle. \label{eq:01} 
\end{align} 
%
Combining \eqref{eq:00} and \eqref{eq:01} completes the proof.
%and applying triangle inequality completes the proof.
\end{proof}  

\subsection{Proof of Proposition \ref{prop:tau}} 

\begin{proof}
We first unpack the numerator in \eqref{eq:tau}:
%
\begin{align}
	\| \phi(\btx) - \bP  \phi(\btx) \|_{\Hc}^2 
	&= \langle \phi(\btx), \phi(\btx) \rangle - 2 \langle \phi(\btx), \bP  \phi(\btx) \rangle + \langle \bP  \phi(\btx), \bP  \phi(\btx) \rangle 
	\\ &= \langle \phi(\btx), \phi(\btx) \rangle -  \langle \phi(\btx), \bP  \phi(\btx) \rangle. \label{eq:0} 
\end{align}	
%
%Note that to arrive at the final equality, we used the properties $\bP' = \bP$ and $\bP^2 = \bP$ given that $\bP$ is an orthogonal projection matrix. 
%
Next, we analyze the second term in \eqref{eq:0}. 
%
Towards this, let us define the (unnormalized) covariance matrix of the mapped features as 
\begin{align} \label{eq:cov} 
	\bSigma = \sum_{i=1}^n \phi(\bx_i) \phi(\bx_i)'
	=  \Phi(\bX)' \Phi(\bX). 
\end{align} 
%
Given that $\bSigma$ is a positive semidefinite matrix, it follows that $\bSigma$ admits an eigendecomposition $\bSigma = \bV \bLambda \bV'$, where $\bV$ is the matrix of eigenvectors and $\bLambda$ is a diagonal matrix of non-negative eigenvalues. 
%
Notably, we can express $\bP$ in terms of $\bV$; namely, $\bP = \bV \bV'$. 
%
Hence, in order to evaluate \eqref{eq:0}, it remains to compute the eigendecomposition of $\bSigma$.

In most settings, however, such a decomposition is intractable given that the dimension of each eigenvector can be arbitrarily large. 
%
Nevertheless, we will show that it is indeed possible to evaluate \eqref{eq:0} via the kernel trick. 
%
To see this, consider the $j$th eigenproblem, i.e., 
\begin{align}
	 \bSigma \bv_j &=  \lambda_j \bv_j. \label{eq:eig}
\end{align} 
Plugging \eqref{eq:cov} into \eqref{eq:eig} and rearranging, we have 
\begin{align}
	\bv_j &= \Phi(\bX)' \left( \frac{\Phi(\bX) \bv_j}{ \lambda_j} \right)
	= \Phi(\bX)' \bw_j, \label{eq:eig2} 
\end{align} 
where $\bw_j = (1/  \lambda_j) \Phi(\bX) \bv_j \in \Rb^n$. 
%
In words, \eqref{eq:eig2} states that the eigenvectors of $\bSigma$ are embedded within the linear subspace spanned by the feature vectors $\phi(\bx_i)$ for $i=1, \dots,n$. 
%
Using \eqref{eq:eig} and the orthonormal property of $\bV$ (i.e., $\bv_j$ has unit norm), observe that 
\begin{align}
	\| \bw_j \|_2^2 &= \frac{1}{\lambda_j^2} \bv_j' \Phi(\bX)' \Phi(\bX) \bv_j = \frac{1}{ \lambda_j^2} \bv_j' (\lambda_j \bv_j) = \frac{1}{\lambda_j}. \label{eq:w_norm} 
\end{align}
%
Moreover, using \eqref{eq:eig} and \eqref{eq:eig2}, we obtain 
\begin{align}
	\Phi(\bX) \Phi(\bX)' \bw_j &= \Phi(\bX) \Phi(\bX)' \left( \frac{1}{ \lambda_j} \Phi(\bX) \bv_j \right) 
	%\\ &= \frac{1}{n \lambda_j} \Phi(\bX) (n \lambda_j \bv_j) 
	\\ &= \Phi(\bX) \bv_j 
	\\ &=  \lambda_j \bw_j. \label{eq:eig3} 
\end{align} 
%
Recalling that $\bK = \Phi(\bX) \Phi(\bX)' \in \Rb^{n \times n}$, we note that \eqref{eq:eig3} suggests that $\bw_j$ corresponds to the $j$th (unnormalized) eigenvector of $\bK$.  
%
As such, it follows that $\bw_j$ can be computed from the eigendecomposition of $\bK$, which is finite-dimensional, and then renormalized to have norm $1/\lambda_j$, as seen from \eqref{eq:w_norm}. 
%
Therefore, we conclude that $\bV = \Phi(\bX)' \bW$, where the $j$th column of $\bW$ corresponds to $\bw_j$. 

Returning to our original task of evaluating \eqref{eq:0}, we find that
\begin{align}
	\langle \phi(\btx), \bP \phi(\btx) \rangle &= \phi(\btx)' \bV \bV' \phi(\btx) 
	\\ &= \phi(\btx)' \Phi(\bX) \bW \bW' \Phi(\bX) \phi(\btx)
	\\ &= \phi(\btx)' \Phi(\bX)' \bW \bW' \Phi(\bX) \phi(\btx); \label{eq:simplify} 
\end{align} 
%
Plugging \eqref{eq:simplify} into \eqref{eq:0} and observing that $\langle \phi(\btx), \phi(\btx) \rangle = k(\btx, \btx)$, we conclude  
\begin{align}
	\| \phi(\btx) - \bP  \phi(\btx) \|_{\Hc}^2 &= k(\btx, \btx) - \langle \bW' \Phi(\bX) \phi(\btx), \bW' \Phi(\bX) \phi(\btx) \rangle.
\end{align} 
This completes the proof. 
\end{proof}




==> content/simulation.tex <==
\newpage
\clearpage 

\section{Calibrated Simulation Studies: Part II} \label{sec:simulations} 
%
The purpose of this section is to continue assessing the relative performances between the mixed intervals and the \HZ~and \VT~specific intervals. 
%
To this end, we consider the California Proposition 99 study of \cite{abadie2}. 
%
Below, we follow the outline described in Section~\ref{sec:simulations.1}. 

% DGP 
{\bf Data generating process.} 
%
We follow the DGP described in Section~\ref{sec:simulations.1}.

% simulation results
{\bf Simulation results.} 
%
We conduct 500 replications of the DGP for the California study.

% prediction errors 
\underline{\em I: Prediction errors.} 
%
Figure~\ref{fig:bias} visualizes the distribution of (normalized) biases and RMSEs for OLS and PCR across all three case studies.  
%
In Table~\ref{table:bias_ca}, we summarize the average biases and root-mean-squared-errors (RMSEs) for the California study. 
%
Similar to the conclusion drawn from Table~\ref{table:bias_rmse}, we find that the true outcome is well approximated by a linear model. 

% ERROR PLOTS
\begin{figure} [!h]
	\centering 
	% 
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/basque.png}
		\caption{Basque Country.} 
		\label{fig:bias_basque} 
	\end{subfigure} 
	%
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/prop99.png}
		\caption{California.} 
	\end{subfigure}
	%
	\begin{subfigure}[b]{0.32\textwidth}
		\centering 
		\includegraphics[width=\linewidth]
		{images/germany.png}
		\caption{W. Germany.} 
	\end{subfigure} 	
	\caption{Distribution of biases across the three case studies. The blue and green distributions correspond to OLS and PCR, respectively. The distributions are visually masked in \ref{fig:bias_basque} due to the large bias gap between OLS and PCR. 
	}
	\label{fig:bias} 
\end{figure} 

% OLS BIAS + RMSE 
\begin{table} [!h]
\centering 
\smaller 
\begin{tabular}{@{}ccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study} 
& \multicolumn{2}{c}{OLS} 
& \multicolumn{2}{c}{PCR}  
\\ 
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& Bias   & RMSE  
& Bias   & RMSE 
\\
\cmidrule(){1-5} 
California
& $0.01$    & $0.08$    
& $0.03$    & $0.03$    
\\ 
\bottomrule
\end{tabular}
\caption{Simulation results in terms of average bias and RMSE for OLS and PCR across 500 replications.}
\label{table:bias_ca}
\end{table} 

% coverage
\underline{\em II: Coverage rates.} 
%
%Tables~\ref{table:ols_ca} and \ref{table:pcr_ca} show the coverage rates for nominal 95\% confidence intervals of OLS and PCR, respectively.
We compute 95\% confidence intervals for the various uncertainty estimators of interest. 
%
Table~\ref{table:ols_ca} shows that the \VT~OLS intervals are degenerate while the mixed OLS intervals match the \HZ~OLS intervals. 
%
Table~\ref{table:pcr_ca} shows that the \HZ~PCR and \VT~PCR intervals undercover while the mixed PCR coverages are closer to the nominal coverage. 
%
These results are in line with our observations in Section~\ref{sec:simulations.1}. 

\begin{table} [!t]
\centering 
\smaller 
\begin{tabular}{@{}ccccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study} 
& \multicolumn{3}{c}{OLS Homoskedastic} 
& \multicolumn{3}{c}{OLS Jackknife}  
\\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
& \HZ   & \VT   & Mixed  
& \HZ   & \VT   & Mixed 
\\
\cmidrule(){1-7} 
California 
% ols
& $0.90$    & $0.00$    & $0.90$ 
& $0.99$    & $0.00$    & $0.99$ 
\\
\bottomrule
\end{tabular}
\caption{Coverage results for nominal 95\% confidence intervals for OLS. We do not report HRK coverage rates as the estimators are not well-defined as per the nonsingularity conditions discussed in Section~\ref{sec:ci.1}. We also do not report the coverage rates for the modified mixed interval as they are equivalent to that of the standard mixed interval. All results are based on 500 simulation replications.}
\label{table:ols_ca}
\end{table}

% PCR COVERAGE
\begin{table} [!t]
\centering 
\smaller 
\begin{tabular}{@{}cccccccccc@{}}
\toprule
\midrule 
\multirow{2}{*}{Case study}  
& \multicolumn{3}{c}{PCR Homoskedastic} 
& \multicolumn{3}{c}{PCR Jackknife}  
& \multicolumn{3}{c}{PCR HRK} 
\\ 
\cmidrule(l){2-4} 
\cmidrule(l){5-7}
\cmidrule(l){8-10}
& \HZ   & \VT   & Mixed     
& \HZ   & \VT   & Mixed  	
& \HZ   & \VT   & Mixed     
\\
\cmidrule(){1-10} 
California 
% pcr 
& $0.73$    & $0.58$    & $0.90$    
& $0.84$    & $0.65$    & $0.94$    
& $0.70$    & $0.57$    & $0.88$    
\\
\bottomrule
\end{tabular}
\caption{Coverage results for nominal 95\% confidence intervals for PCR. All results are based on 500 simulation replications.}
\label{table:pcr_ca}
\end{table}


